An Axiomatic Theory of Provably-Fair Welfare-Centric Machine Learning

We address an inherent difficulty in welfare-theoretic fair machine learning by proposing an equivalently axiomatically-justified alternative and studying the resulting computational and statistical learning questions. Welfare metrics quantify overall wellbeing across a population of one or more groups, and welfare-based objectives and constraints have recently been proposed to incentivize fair machine learning methods to produce satisfactory solutions that consider the diverse needs of multiple groups. Unfortunately, many machine-learning problems are more naturally cast as loss minimization tasks, rather than utility maximization, which complicates direct application of welfare-centric methods to fair machine learning. In this work, we define a complementary measure, termed malfare, measuring overall societal harm (rather than wellbeing), with axiomatic justification via the standard axioms of cardinal welfare. We then cast fair machine learning as malfare minimization over the risk values (expected losses) of each group. Surprisingly, the axioms of cardinal welfare (malfare) dictate that this is not equivalent to simply defining utility as negative loss. Building upon these concepts, we define fair-PAC (FPAC) learning, where an FPAC learner is an algorithm that learns an $\varepsilon$-$\delta$ malfare-optimal model with bounded sample complexity, for any data distribution, and for any (axiomatically justified) malfare concept. Finally, we show broad conditions under which, with appropriate modifications, standard PAC-learners may be converted to FPAC learners. This places FPAC learning on firm theoretical ground, as it yields statistical and computational efficiency guarantees for many well-studied machine-learning models, and is also practically relevant, as it democratizes fair ML by providing concrete training algorithms and rigorous generalization guarantees for these models

==> paper/linearfig.tex <==
TODO: FILE NOT USED; EMBEDDED IN CONTENT

\begin{tikzpicture}[line cap=round]

\clip (-3, -1.44) rectangle (8, 3.4);

\onslide<2,4->{
\node at (0.333, 1.69) {\textcolor{red}{\gone}};
\node at (-0.1, 0.1) {\textcolor{red}{\gone}};
\node at (-1.01, 1) {\textcolor{red}{\gone}};
\node at (-2.2, 3) {\textcolor{red}{\gone}};
\node at (-2.8, -0.5) {\textcolor{red}{\gone}};

\node at (0, -0.456) {\textcolor{blue}{\gone}};
\node at (1, 1.1) {\textcolor{blue}{\gone}};
\node at (2.3, 2.1) {\textcolor{blue}{\gone}};
\node at (3.1, -0.5) {\textcolor{blue}{\gone}};
}

\onslide<3,4->{
\node at (-0.69, 0.5) {\textcolor{red}{\gtwo}};
\node at (-2.08, 1.87) {\textcolor{red}{\gtwo}};
\node at (0.146, -1.24) {\textcolor{red}{\gtwo}};
\node at (1.824, 0.863) {\textcolor{red}{\gtwo}};

\node at (0.42, 2.81) {\textcolor{blue}{\gtwo}};
\node at (2.1, 3.08) {\textcolor{blue}{\gtwo}};
\node at (2.75, 0.6) {\textcolor{blue}{\gtwo}};
}

%Errors:
\onslide<5->{
\node[draw,circle,black,thick] at (1.824, 0.863) {\textcolor{red}{\gtwo}};
\node[draw,circle,black,thick] at (0, -0.456) {\textcolor{blue}{\gone}};
}

\node[rectangle,draw=black] at (5.5, 2) {
\begin{tabular}{cl}
\textcolor{red}{$\blacksquare$} & Class A \\
\textcolor{blue}{$\blacksquare$} & Class B \\
\textcolor{purple}{\bf |} & Linear Separator \\%[-0.4cm]
\onslide<2,4->{\gone & Group 1} \\
\onslide<3,4->{\gtwo & Group 2} \\
\end{tabular}
};

%\draw[purple] (-0.1, -1) -- (0.5, 3);


\onslide<2,4->{
\begin{scope}[rotate=-25]
\draw[purple,thick,dashed] (0, -4) -- (0, 4);
%\draw[purple,thick,dashed] (0, -2) -- (0, 2);
%\node at (0, -2.5) {\color{purple}\bf\gone};
\end{scope}
}

\onslide<3,4->{
\begin{scope}[rotate=47.5]
%\draw[purple,thick,dashed] (4.3, -4) -- (4.3, 4);
%\draw[purple,thick,dashed] (2.15, -2) -- (2.15, 2);
\draw[purple,thick,dashed] (2.15, -4) -- (2.15, 4);
%\node at (0, -2.5) {\color{purple}\bf\gtwo};
\end{scope}
}

\onslide<5->{
\begin{scope}[rotate=18]
%\draw[purple,thick] (2.2, -4) -- (2.2, 6);
%\draw[purple,thick] (1.1, -2) -- (1.1, 3);
\draw[purple,thick] (1.1, -4) -- (1.1, 4);
%\node at (1.1, -2.5) {\color{purple}\bf\gone\gtwo};
\end{scope}
}


\end{tikzpicture}


==> paper/misc.tex <==


{

Attempted diffEQ power mean proof:


\if 0 %Many failed attempts:


\[
ax 1-5 \implies \ln(F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))])) = \ln(\alpha F(\Expect_{\omega \distributed \wv}[f_{p}(\lv(\omega))])) = \ln(\alpha) + \ln( F(\Expect_{\omega \distributed \wv}[f_{p}(\lv(\omega))]))
\]

Now we do some differential equations.
\[
\frac{\partial}{\partial \alpha} \ln(F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))])) = \frac{1}{F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))])} \cdot \frac{\partial}{\partial \alpha} F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))])
\]
\[
\frac{\partial}{\partial \alpha} \ln(\alpha) + \ln( F(\Expect_{\omega \distributed \wv}[f_{p}(\lv(\omega))])) = \frac{1}{\alpha}
\]

Thus
\[
\frac{\partial}{\partial \alpha} F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))]) = \frac{F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))])}{\alpha}
\]

We now consider the case $p > 0$.  Substituting $f_{p}(u) = u^{p}$, we have
\[
\frac{\partial}{\partial \alpha} F(\alpha^{p} \Expect_{\omega \distributed \wv}[\lv^{p}(\omega))])
 = \frac{F(\alpha^{p}\Expect_{\omega \distributed \wv}[\lv^{p}(\omega)])}{\alpha}
\]

Take $q \doteq \Expect_{\omega \distributed \wv}[\lv^{p}(\omega)]$.  We have
\[
\frac{\partial}{\partial \alpha} F(\alpha^{p} q)
 = \frac{F(\alpha^{p}q)}{\alpha}
\]

Now, apply the chain rule again:
\[
\frac{\partial}{\partial \alpha} F(\alpha^{p} q) = \dots
\]

Now, make substitution $x = \alpha^{p}q$.  We have
\[
\frac{\partial}{\partial \alpha} F(x) = \frac{F(x)}{\sqrt[p]{\nicefrac{x}{q}}} \enspace.
\]


\todo{this shows power mean have this property, not the other way around?} Now, take $G(u) = \sqrt[p]{u}$, and note that $\frac{\partial}{\partial \alpha} G(\alpha^{p}q) = \frac{G(\alpha^{p} q)}{\alpha}$





\todo{NEW ATTEMPT:}
\[
\frac{\partial}{\partial \alpha} F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha \lv(\omega))])
 = \frac{\partial}{\partial \alpha} F(\alpha^{p}\Expect_{\omega \distributed \wv}[ \lv^{p}(\omega))])
 = \frac{\partial}{\partial \alpha} F(\alpha^{p}q)
 = F'(\alpha^{p}q) p \alpha^{p-1}q \enspace.
\]

Consequently, we have
\[
F'(\alpha^{p}q) 
 = \frac{F(\alpha^{p}q)}{p\alpha^{p}}
 \implies \frac{F(\alpha^{p}q)}{F'(\alpha^{p}q)} = qp\alpha^{p}
\]

Now we hope for a logarithmiracle
\[
\ln(F(\alpha^{p}q)) - \ln(F'(\alpha^{p}q)) = \ln(qp\alpha^{p})
\]




\todo{or try:}

Now substitute:
\[
\frac{F(\sqrt[p]{\alpha^{p}q})}{F'(\sqrt[p]{\alpha^{p}q)}} = \sqrt[p]{p\alpha^{p}}
\]

\todo{Q above!}

Now, make substitution $x = \alpha^{p}q$.  We have
\[
F'(x) = \frac{F(x)}{x} \implies \frac{F(x)}{F'(x)} = x \enspace.
\]

\todo{wrong:} This tells us (by Clairaut's equation) that $F(x) = c x$.  Substituting back gives us
\[
F(\alpha^{p}q) = c \alpha^{p}q
\]


\todo{This is fine, but another log should clean it up better?}

Now, note that the only $F$ s.t. $\frac{\partial}{\partial \alpha} F(\alpha^{p}q) = \frac{F(\alpha^{p}q)}{\alpha}$

\todo{By ???, the only soln to this diff eq is.}

\todo{bad expect $p$ subscript...}




\todo{Another try with the inverse:}

Suppose $\lv(\cdot) = 1$, and take $\Mean(\lv; \wv) = c$.

For all $p \in (0, \infty)$, we have:
\[
c = \Mean(\lv; \wv) = F(\Expect_{\omega \distributed \wv}[f_{p}(\lv(\omega))] = F(1)
\]

\[
\alpha c = \alpha\Mean(\lv; \wv) = \Mean(\alpha\lv; \wv) = F(\Expect_{\omega \distributed \wv}[f_{p}(\alpha\lv(\omega))] = F(\alpha^{p})
\]

Now, we apply $F^{-1}$ to both sides of both equations and divide \todo{check / 0}:



\if 0
\[
F^{-1}\Mean(\lv; \wv) = \Expect_{\omega \distributed \wv}[f_{p}(\lv(\omega))]
\]

\[
F^{-1}\alpha\Mean(\lv; \wv) = \alpha^{p}\Expect_{\omega \distributed \wv}[f_{p}(\lv(\omega))]
\]

\[
\frac{F^{-1}(\alpha\Mean(\lv; \wv))}{F^{-1}\Mean(\lv; \wv)} = \alpha^{p}
\]
\[
F^{-1}(\alpha q) = \alpha^{p} q \implies F^{-1}(u) = u^{p}
\]

\fi

\[
\frac{F^{-1}(\alpha c)}{F^{-1}(c)} = \alpha^{p}
\]





\todo{With inverse and unit scale:}
\fi



}


==> paper/pac.tex <==

\todo{As in original document.}

\todo{Claim: Atk hard to estimate: \url{https://ideas.repec.org/p/iza/izadps/dp763.html}.}

\todo{Submit to EC? new letter for $n$?}

We first illustrate the ease of which $p$-power means can be estimated, in contrast to the standard additive welfare formulations.

\begin{lemma}[Statistical Estimation]%  (Range Only)]
\label{lemma:stat-est}
Suppose probability distribution $\ProbDist$, population-mean $\Mean$ obeying \emph{monotonicity}, sentiment value function $\lv$ such that, given functions $f_{\omega}$, we have $\lv(\omega) = \Expect_{x \distributed \ProbDist}[f_{\omega}(x)]$, sample $\bm{x} \distributed \ProbDist^{m}$, and \emph{empirical sentiment value estimate} $\hat{\lv} \doteq \EExpect_{x \in \bm{x}}[f_{\omega}(x)]$.
If it holds with probability at least $1 - \delta$ that $\forall \omega: \, \lv'(\omega) - \epsv(\omega) \leq \lv(\omega) \leq \lv'(\omega) + \epsv(\omega)$, then with said probability, we have
\[
\Mean_{p}(\bm{0} \vee (\hat{\lv} - \epsv); \wv)
  \leq \Mean_{p}(\hat{\lv}; \wv)
  \leq \Mean_{p}(\hat{\lv} + \epsv; \wv)
  \enspace,
\]
where $\bm{a} \vee \bm{b}$ denotes the (elementwise) minimum.
\end{lemma}
\begin{proof}
This result follows from the assumption, and the \emph{monotonicity} axiom (i.e., adding or subtracting $\epsv$ can not decrease or increase the power mean, respectively).
The minimum with $0$ on the LHS is required simply because by definition, sentiment values are nonnegative, and $\Mean_{p}$ is in general undefined with negative inputs.
\todo{2-sided variant?}
\end{proof}

\todo{fwd ref codecs?}


We now reify this result, applying the well-known Hoeffding and Bennett bounds to show concentration and derive an explicit form for $\epsv$.

\begin{corollary}[Statistical Estimation with Hoeffding and Bennett Bounds]% (Range Only)]
\label{coro:stat-est}
Suppose fair power-mean Malfare $\Malfare(\dots)$ (i.e., $p \geq 1$), \emph{loss function} $\LossFunction: \X \to [0, \frange]$, $\lv \in [0, \frange]^{n}$ s.t. $\lv_{i} = \Expect_{\ProbDist_{i}}[\LossFunction]$, samples $\bm{x}_{i} \distributed \ProbDist_{i}^{m}$ and $\hat{\lv}_{i} = \frac{1}{m}\sum_{j=1}^{m} \LossFunction(\bm{x}_{i,j})$.
Then with probability at least $1 - \delta$ over choice of $\bm{x}$,
\[
\abs{ \Mean_{p}(\lv; \wv) - \Mean_{p}(\hat{\lv}; \wv) } \leq \frange\sqrt{\frac{\ln \frac{2n}{\delta}}{2m}} \enspace.
  %Bennett:
  %? + \sqrt{\frac{2 v? \ln \frac{n}{\delta}}{m}}
\]
Alternatively, again with probability at least $1 - \delta$ over choice of $\bm{x}$, we have
\[
\abs{ \Mean_{p}(\lv; \wv) - \Mean_{p}(\hat{\lv}; \wv) } \leq \frac{\frange\ln \frac{2n}{\delta}}{3m} + \sup_{i \in 1, \dots, n} \sqrt{\frac{2\Var_{\ProbDist_{i}}[\LossFunction] \ln \frac{2n}{\delta}}{m}} \enspace.
  %Bennett:
  %? + \sqrt{\frac{2 v? \ln \frac{n}{\delta}}{m}}
\]
\end{corollary}
\begin{proof}
This result is a corollary of \cref{lemma:stat-est}, applied to $\epsv$, where we note that for $p \geq 1$, by \cref{thm:pow-mean-prop}~item~\ref{thm:pow-mean-prop:contraction} (contraction)
it holds that
\[
\Mean_{p}(\hat{\lv} + \epsv; \wv) \leq \Mean_{p}(\hat{\lv}; \wv) + \norm{\epsv}_{\infty} \ \& \ \Mean_{p}(\bm{0} \vee (\hat{\lv} - \epsv); \wv) \leq \Mean_{p}(\hat{\lv}; \wv) - \norm{\epsv}_{\infty} \enspace.
\]

Now, for the first bound, note that we take $\epsv_ {i} \doteq \frange\sqrt{\frac{\ln \frac{2n}{\delta}}{2m}}$, and by Hoeffding's inequality and the union bound, for $\Omega = \{1, \dots, n\}$, we have $\forall \omega: \, \lv'(\omega) - \epsv(\omega) \leq \lv(\omega) \leq \lv'(\omega) + \epsv(\omega)$ with probability at least $1 - \delta$.
The result then follows via the \emph{power-mean contraction} (\cref{thm:pow-mean-prop} item \ref{thm:pow-mean-prop:contraction}) property.

Similarly, for the second bound, note that we take $\epsv_ {i} \doteq \frac{\frange\ln \frac{2n}{\delta}}{3m} + %\sup_{i \in 1, \dots, n}
\sqrt{\frac{2\Var_{\ProbDist_{i}}[\LossFunction] \ln \frac{2n}{\delta}}{m}}$, which this time follows via Bennett's inequality and the union bound.
Now, we again apply \cref{lemma:stat-est}, noting that $\Mean(\epsv) \leq \Mean_{\infty}(\epsv) = \norm{\epsv}_{\infty}$ (by \emph{power-mean monotonicity}, \cref{thm:pow-mean-prop:mono} item \ref{thm:pow-mean-prop:mono}), and the rest follows as in the Hoeffding case.
% and the rest is as with the Hoeffding case. % (note that here thus the \rhs{} is $\norm{\epsv}_{\infty}$).
%\todo{improvement: 1 side is direct by concavity convextity: $2n$ could be $n+1$?}
\end{proof}
%The above bound is a straightforward consequence of Hoeffding's inequality; similar variance-sensitive bounds can be shown with Bennett's inequality, and uniform convergence bounds with Rademacher averages.


As \cref{coro:stat-est} follows directly from \cref{lemma:stat-est}, with Hoeffding and Bennett inequalities applied to derive $\epsv$ bounds, similar results are immediately possible with arbitrary concentration inequalities.
In particular, we can show \emph{data-dependent} bounds may be shown, e.g., with empirical Bennett bounds, removing dependence on \emph{a priori known variance}.
\ifthesis
In particular, we may apply \cref{thm:firstbound} to bound $\epsv$, either elementwise (over groups) with a \emph{union bound}, or jointly, if the loss functions for each group may be combined into a single function family.
\todo{backref rade bounds}
\fi


Furthermore, note that while these bounds may be used for \emph{evaluating} the welfare or malfare of a \emph{particular} classifier or mechanism (through $\lv$ and $\hat{\lv}$), they immediately extend to \emph{learning} over a \emph{finite family} via the union bound.
Much like in standard statistical learning theory, the exponential tail bounds of \cref{coro:stat-est} allow the family to grow \emph{exponentially}, at \emph{linear} cost to sample complexity.
Also as in standard uniform convergence analysis (generally discussed in the context of \emph{empirical risk minimization}), we can easily handle infinite hypothesis classes and obtain much sharper bounds by considering \emph{uniform convergence bounds} over the family, i.e., with Rademacher averages and appropriate concentration-of-measure bounds.

\todo{eval vs learning; union bound.}


%, and similarly with uniform convergence and Rademacher averages, to show such bounds over a \emph{class} of sentiment vectors (i.e., each describing how a classifier impacts all groups).%  dependence on $n$.
In all cases, these bounds provide further justification for using the \emph{power-mean} over the \emph{additively separable} form, as it is substantially harder to achieve comparable bounds on
%\[
%\Mean_{p}^{p}(\lv; \wv) \enspace,
%\]
$\Mean_{p}^{p}(\lv; \wv)$,
due to the increased difficulty of controlling the \emph{range} and \emph{Lipschitz constant} of these quantities.
Of course, as power-mean bounds imply bounds on the additively-separable form (and vice-versa), we recommend working with power means, and then converting back to the additively separable form (if so desired).

%Variance-sensitive bounds are particularly irksome, as the variance proxies of interest are $\Var[\lv^{p}](\omega)$, rather than simply $\Var[\lv(\omega)]$.

\todo{It's about balancing interpretability and estimability; I think we're better on both counts.  Changing $p$ doesn't change interpretation (as much). Plot of normalized vs denorm?}

\subsection{Characterizing Fair Learnability}
\label{sec:est-learn:pac}

We now characterize a notion of \emph{fair-learnability} in machine learning, reminiscent of standard \emph{\underline{p}robably \underline{a}pproximately \underline{c}orrect (PAC) learning} guarantees of \citet{valiant1984theory}.
In particular, we generalize to our definition to \emph{arbitrary supervised learning problems} (i.e., beyond binary classification with 0-1 loss), and to \emph{agnostic learning} problems, and settings with non-zero Bayes risk (i.e., so-called \emph{noisy} problems, where $x$ does not uniquely determine $y$).
Following the original conception of PAC-learnability, we also include \emph{computational considerations} in our definition; i.e., it is predicated on the existence of an efficient training algorithm.
Some authors, e.g., \citet[Definition 3.1]{shalev2014understanding} and \citet[Definition 14.9]{mitzenmacher2017probability}, consider \emph{computational complexity} a separate issue, and instead define PAC-learnability as requiring polynomial \emph{sample complexity}, though doing so leads to a breakdown in the learnability hierarchy (i.e., finite VC dimension, PAC-learnability, and agnostic PAC-learnability become equivalent, see \citet[thm.~6.7]{shalev2014understanding}).
%  our definition \todo{generalized beyond classification to  agnostic.}
%In our definition, we assume 
Our definition requires a computationally efficient training procedure, but this requirement may be removed by assuming a training oracle.
Following our definition, we show sufficient conditions under which an algorithm is fair-PAC-learnable.
%Our notion of fair PAC learnability

\todo{Mutual unsatisfiability ctrnt; naive idealism; reality a resource allocation}




 


For context, we first present a generalized notion of PAC-learnability, which we then generalize to fair-PAC-learnability.
In the realizable case, we assume $\exists h^{*} \in \HC$ s.t.\ $\Risk_{\ProbDist}(h^{*}; \loss) = 0$, which restricts the space of possible probability distributions.
For reasons that shall later be made clear, we consider only the \emph{agnostic learning case}, where this assumption is dropped.
%All of our results are presented in the agnostic case (i.e., we don't constrain the instance distribution such that $\HC$ contains a 0-risk solution).

%\draftnote{TODO: ERISK LOSS; agnostic term}


\begin{definition}[Agnostic PAC-Learnability]
\label{def:pac}
%An algorithm $\PACAlgo$ is said to be 
Suppose a \emph{hypothesis class} $\HC \subseteq \X \to \Y$, and \emph{loss function} $\LossFunction: \Y \times \Y \to \R_{0+}$.
We say $\HC$ is \emph{PAC-learnable} \wrt{} $\LossFunction$ if $\exists$ a (randomized) algorithm $\PACAlgo$, such that $\forall$:
\todo{poly computable}
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item instance distributions $\ProbDist$ over $\X \times \Y$;
\item additive approximation error $\varepsilon > 0$;
\item failure probability $\delta \in (0, 1)$;
\end{enumerate}
it holds that $\PACAlgo$ can identify a hypothesis $\hat{h} \in \HC$ such that
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\PACAlgo$ has $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta})$ expected sample complexity;
%\emph{polynomial} (in $n$, $\nicefrac{1}{\varepsilon}$, and $\nicefrac{1}{\delta}$) expected time complexity.%, space, entropy, and sample complexity (i.e., requires polynomially bounded computational, memory, randomness, and training instances);
\item with probability at least $1 - \delta$ (over randomness of $\PACAlgo$), $\hat{h}$ obeys
\[
\Expect_{(x, y) \distributed \ProbDist} \bigl[ \loss(y, \hat{h}(x)) \bigr] \leq \inf_{h^{*} \in \HC} \Expect_{(x, y) \distributed \ProbDist} \bigl[\loss(y, h^{*}(x)) \bigr] + \varepsilon \enspace.
\]
\todo{RISK DEF.}
\todo{$\hat{h}$ is \emph{measurable} and \emph{computable} in poly time?}
\todo{risk notation?}
\end{enumerate}


\end{definition}

Note that this substantially differs from the original presentation of PAC-learning \citep{valiant1984theory}, which handles only \emph{binary classification} with $0$-$1$ loss, and we consider PAC-learnability \emph{\wrt} a particular (arbitrary) loss function.
%In particular, note that our concept of fair-PAC-learnability is parameterized by both the \emph{hypothesis class} $\HC$ and \emph{loss function} $\loss$, 
Note that PAC-learnability is a property of both $\HC$ and $\loss$, and we can not hope for uniform guarantees over \emph{arbitrary loss functions}.\footnote{Trivially, for infinite $\X$, $\Y = \pm 1$ (binary classification), we have that $\HC = \Y^{\X} = \X \mapsto \Y$\todo{check notation} is not PAC-learnable \wrt{} 0-1 loss; thus requiring uniformity over choice of $\HC$ would leave the class of fair-PAC-learnable models woefully vacuous.
Similarly for any loss $\LossFunction$ s.t.\ the problem is unrealizable, taking $\LossFunction'(y, \hat{y}) \doteq \alpha\LossFunction(y, \hat{y})$ is equivalent to taking $\varepsilon' \doteq \nicefrac{\varepsilon}{\alpha}$, thus precluding polynomial dependence on $\nicefrac{1}{\varepsilon}$ except in the realizable case; thus again requiring uniformity over choice of $\loss$ greatly restricts the concept of fair-PAC-learnability.}
\todo{Also agnostic.}

\todo{Following the convention of \citep{shalev2014understanding,mitzenmacher2017probability}, \dots}

We now generalize PAC-learnability to fair-PAC-learnability.


\begin{definition}[Fair Agnostic PAC-Learnability]
\label{def:fair-pac}
%An algorithm $\PACAlgo$ is said to be 
Suppose a \emph{hypothesis class} $\HC \subseteq \X \to \Y$, and \emph{loss function} $\LossFunction: \Y \times \Y \to \R_{0+}$.
We say $\HC$ is \emph{fair PAC-learnable} \wrt{} \emph{group count} $n$ and $\LossFunction$ if $\exists$ a (randomized) algorithm $\PACAlgo$, such that $\forall$:
\todo{poly computable}
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
%\item group count $n$;
\item instance distributions $\ProbDist_{1:n}$ over $(\X \times \Y)^{n}$;
\item group weights measure $\wv$ over $\{1, \dots, n\}$;
\item malfare concept $\Malfare(\dots)$ satisfying axioms 1-7 and \ref{def:cardinal-axioms:apd};\todo{macro for axs.}
\item additive approximation error $\varepsilon > 0$;
\item failure probability $\delta \in (0, 1)$;
\end{enumerate}
it holds that $\PACAlgo$ can identify a hypothesis $\hat{h} \in \HC$ such that
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\PACAlgo$ has $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta})$ expected sample complexity. %\emph{polynomial} (in $\nicefrac{1}{\varepsilon}$, and $\nicefrac{1}{\delta}$) expected time complexity.%, space, entropy, and sample complexity (i.e., requires polynomially bounded computational, memory, randomness, and training instances);
\item with probability at least $1 - \delta$ (over randomness of $\PACAlgo$), $\hat{h}$ obeys
\[
\Malfare\left(i \mapsto \biggl( \Expect_{(x, y) \distributed \ProbDist_{i}} \bigl[ \loss(y, \hat{h}(x)) \bigr] \biggr); \wv \right) \leq \inf_{h^{*} \in \HC} \Malfare \left(i \mapsto \biggl(\Expect_{(x, y) \distributed \ProbDist_{i}} \bigl[\loss(y, h^{*}(x)) \bigr] \biggr); \wv \right) + \varepsilon \enspace.
\]
\todo{$\hat{h}$ is \emph{measurable} and \emph{computable} in poly time?}
\todo{risk notation?}
\end{enumerate}
%\draftnote{I think it's slightly weaker to suppose (fix) $n$, rather than require $\forall n$, but it might be a cleaner definition?  I don't have an example that's fair-PAC learnable one way but not the other.}
%\draftnote{Similarly, is there a difference between $\forall \Malfare$ and assuming specific $\Malfare$?}
\end{definition}

\todo{Again efficient?}

\todo{Note $n=1$ coincides with ...  uniform over $n$}

Note that this definition is extremely specific, and perhaps our axiomatization and all previous relevant results should be viewed as leading up to it.
We first discuss a few highly precise definitional choices, and explain why they are equivalent to classes that perhaps seems broader or more specific at first glance.
We then discuss the \emph{motivations} for particular assumptions, and how they relate to our previous analysis of the cardinal welfare axioms and their statistical estimation properties.
First note that assuming an instance distribution $\ProbDist_{1:n}$ over $(\X \times \Y)^{n}$ is important to remain general over sampling strategies.
In many cases, each marginal distribution $\ProbDist_{i}$ is available separately, and we sample from them \emph{independently}, however in some learning problems, it may make more sense to sample in a dependent manner\todo{game theory; fwd ref to codecs}.
As the definition is not sensitive to \emph{polynomial} complexity changes, being unable to directly sample the marginal distributions is inconsequential.
%Due to the \emph{polynomial dependence on and neither the sample nor time complexity of processing vector samples causes any issues.
\todo{restore time complexity stuff}
\if 0
Another key choice is the requirement of polynomial expected time complexity of $\PACAlgo$.
As a is a randomized algorithm, $\PACAlgo$ it is thus able to sample an expected polynomial amount of entropy, and sample an expected polynomial number of training instances.
These bounds may be converted to high probability or absolute guarantees (at polynomial cost to $\delta$), and similarly, it is also possible to control space complexity, as $\PACAlgo$ doesn't benefit from using a superpolynomial amount of memory.
%Perhaps most importantly from a machine learning perspective it also requires polynomial sample complexity. To
Note also that we assume only that $\PACAlgo$ is \emph{polynomial} in $\nicefrac{1}{\varepsilon}$ and $\nicefrac{1}{\delta}$, though by standard properties of ubiquitous concentration inequalities and concentration of measure phenomena, we almost always expect dependence on $\frac{1}{\varepsilon^{2}}$ and $\smash{\sqrt{\ln\mathsmaller{\frac{1}{\delta}}}}$.
%log 1 of her Delta But we leave the form polynomial so as to simplify the statement and analysis.
\fi


\todo{explain \emph{measurable} and \emph{computable}}


We now discuss the deeper motivation and consequences of \cref{def:fair-pac}
%In contrast, 
Fair-PAC-learnability must hold \emph{uniformly} over the choice of \emph{instance distributions} $\ProbDist_{1:n}$; i.e., the concept is inherently \emph{distribution-free}, in the sense that we require a fair algorithm to be able to (agnostically) learn fairly under any circumstances.
To this end we also require uniformity over \emph{fairness concepts} (item 2; choice of $\wv$, and item 2; choice of $\Malfare(\cdot; \wv)$); consequently, (upper-bounds to) time, space, entropy, and sample complexity must hold \emph{for all}\footnote{Note that by continuity, fair-PAC-learnability implies learnability with $\Malfare_{\infty}(\cdot; \wv)$, by taking $\lim_{p \to \infty}$, although, strictly speaking $\Malfare_{\infty}(\dots)$ fails to meet the continuity axiom.} $p \geq 1$, i.e., they \emph{may not} depend on $p$.
This is perhaps our strongest use of the \emph{unit scale} and \emph{multiplicative linearity} axioms, without which welfare and malfare functions may be arbitrarily scaled and monotonically transformed.%
\footnote{If, for instance, we were to instead require uniformity over the set of malfare functions $\{ \Malfare_{p}^{p}(\cdot; \wv) \mid p \geq 1 \}$, \todo{i.e., the \emph{additively separable form}}, then risk value $\lv(i) \geq 1$ would explode $\lim_{p \to \infty}\Malfare_{p}^{p}(\lv; \wv) = \infty$\todo{weird notation}, and similarly, if $\lv$ is uniformly bounded above by some $B < 1$, $\lim_{p \to \infty}\Malfare_{p}^{p}(\lv; \wv) = 0$ (i.e., everything becomes learnable).}
From our statistical bounds (\cref{lemma:stat-est}),\todo{better ref} we see that learning becomes statistically more challenging for as $p$ increases, due to dependence on $p$-norms and monotonicity in $p$ of $\Malfare_{p}(\cdot; \wv)$, but statistical learning theory is well-equipped to handle even the limiting case of $p = \infty$.
We soon reify this definition by showing highly generic conditions under which classifiers guarantee fair PAC-learnability.


\todo{key idea; change interpretation of welfare to get good behavior.}

\todo{computation of $\hat{h}$? polytime req? bounded loss discussion? depends on $\X, \Y$ universes?}


\paragraph{Fair PAC-learning and computational efficiency}
Note that we specifically assume \emph{fixed $n$}, and in the case of $n=1$, the definition coincides with that of (agnostic) PAC-learnability.
Furthermore, if we wish to consider \emph{computational efficiency}, we may strengthen condition 1 to ``$\PACAlgo$ has $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta})$ expected \emph{time} complexity.''
We term this stronger requirement \emph{efficient fair-PAC-learnability}, following the convention of \citep{shalev2014understanding,mitzenmacher2017probability}.
This convention is convenient, as we shall see that additional conditions are required to show efficiency, so we may distinguish between \emph{sample-efficient} and \emph{computationally efficient} fair learning algorithms.
An even stronger requirement would be to require $\PACAlgo$ to work uniformly over choice of $n$, and require ``$\PACAlgo$ has $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, n)$ expected \emph{time} complexity.''\todo{discuss?}

\paragraph{A note on realizability}
The natural generalization of realizable PAC-learning to fairness is to assume $\exists h^{*} \in \HC$ s.t.\ $\forall i \in \{1, \dots, n\}: \, \Risk_{\ProbDist_{i}}(h^{*}; \loss) = 0$, in which case no real tradeoffs exist, as all groups may be perfectly satisfied simultaneously.
This $h^{*}$ is thus optimal for any malfare concepts satisfying axioms 1-7 and \ref{def:cardinal-axioms:apd}, and may be identified via (standard) PAC-learning over the mixture distribution $\ProbDist_{1:n}$, thus realizable \emph{fair} PAC-learning reduces to realizable PAC-learning.
The concept is also philosophically uninteresting, as \emph{scarcity begets conflict}, and only then must fairness-sensitive tradeoffs occur.
We thus consider only \emph{agnostic learning}, wherein no such mutual satisfiability assumption is made.
\todo{detail:
This is uninteresting in the context of fairness, as it implies a single $h^{*}$ is optimal for all malfare concepts satisfying axioms 1-7 and \ref{def:cardinal-axioms:apd}, in which case it's immediately clear that minimizing $\Malfare_{1}(\cdot)$, which is equivalent to minimizing risk over the mixture of $\ProbDist_{1:n}$, is sufficient, thus in the realizable case, PAC-learnability and fair-PAC learnability coincide.
}

\paragraph{Sufficient conditions for fair PAC-learnability}
\todo{necessary conds? PAC is obvious?}
\todo{More of a meta-thm? why not thm then coros for vc / loss functions / covering concepts}
As noted by \citep{blumer1989learnability}, PAC-learnability and finite VC-dimension \citep{vapnik1968uniform} are essentially equivalent (subject to basic regularity conditions).\todo{Cite VC}
We now extend this analogy to fair-PAC-learning.
\todo{consult blumer for computation details?}
\todo{cite VC?  Describe earlier in thesis?}
%
\begin{theorem}[Fair PAC-Learning with Vapnik-Chervonenkis Classes and Covering Numbers]
\label{thm:fair-covering}
Suppose $\HC$ has finite VC-dimension $d$, and the \emph{projection} of $\HC$ onto $\bm{x} \in \X^{m}$ can be enumerated in $\Poly(m)$ time (wherein $d$ is a constant).
Then $\HC$ is fair-PAC-learnable.

Furthermore, suppose generic $\HC \subseteq \X \to \Y$, $\loss \in \Y \times \Y \to [0, 1]$, and assume that\todo{Scaling?}
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\Y$ is a set of diameter $D_{\Y}$, and $\loss$ is $\lambda_{\loss}$-Lipschitz continuous;
\item the $\ell_{2}$ covering number%
\footnote{The reader is invited to consult \citep{anthony2009neural} for an encyclopedic overview of various covering numbers and their applications to statistical learning theory.}
$\mathcal{N}(\HC, \bm{x}, \gamma) \in \Poly(m, \nicefrac{1}{\gamma})$;
\item a \emph{$\gamma$-precision cover} $\mathcal{C}(\HC, \bm{x}, \gamma)$ of size $\LandauO(\mathcal{N}(\HC, \bm{x}, \gamma))$ may be enumerated in $\Poly(m, \nicefrac{1}{\gamma})$ time.
\end{enumerate}
Then $\HC$ is efficiently fair-PAC-learnable.
Items (1) and (2) are sufficient to show that $\HC$ is fair-PAC learnable; (3) is required only to show \emph{efficiency}.
%
\todo{cite / define covering}
%
\todo{Could start with cover of loss family?}
%
\end{theorem}
\begin{proof}[Proof Sketch]
%Proof soon-to-appear in upcoming work.
%I present a proof-sketch here:
%
First, note that the Vapnik-Chervonenkis conditions on $\HC$ immediately imply that, given samples $\bm{x}_{1:n}$, each of size $m$, each covering number $\mathcal{N}(\HC, \bm{x}_{i}, \gamma) \in \Poly(m, \frac{1}{\gamma}) \leq \sum_{i=1}^{d} \binom{m}{i} \leq m^{d}$, by the Sauer-Shelah lemma,\todo{cite} where the VC-dimension $d$ is \emph{constant} (\wrt~fixed $\HC$), and also, by assumption, this cover may be enumerated in $\Poly(m) = \Poly(m, \nicefrac{1}{\gamma})$ time.
The first case thus reduces to a special case of the second.

I now sketch a proof of the general case.
We first take \emph{cover precision} $\gamma \doteq \frac{\varepsilon}{3D_{\Y}\lambda_{\loss}}$\todo{/range}.
We then show that, taking $\hat{h}$ to be the EMM solution \wrt{} \emph{a cover} of this precision, and $\tilde{h}$ to be the exact EMM solution \wrt{} \emph{all of $\HC$}, it holds that the empirical malfare of $\hat{h}$ does not exceed that of $\tilde{h}$ by more than $\frac{\varepsilon}{3}$.
We then apply standard covering-number bounds on Rademacher averages to show that a (polynomial) sufficient $m$ exists to guarantee $\tilde{h}$ generalizes with $\frac{2\varepsilon}{3}$-$\delta$ malfare error guarantees.
In particular, by the Dudley discretization method, a $\frac{\varepsilon}{3}$ \emph{discretization error} term appears, and we set $m$ such that a $\frac{\varepsilon}{3}$ covering number term appears, for a total of $\frac{2\varepsilon}{3}$.
Combining these bounds on the \emph{optimization} and \emph{approximation} errors yields the desired additive $\epsilon$-$\delta$ guarantees.

Note that (3) implies that the cover may be efficiently enumerated, thus guaranteeing polynomial time complexity.
%
%
\todo{give general case; handle range.}
%
\if 0
\todo{what is $m$?  Sketch p1 is good.}
First, note that the Vapnik-Chervonenkis conditions on $\HC$ immediately imply $\dots \leq \sum \dots \leq m^{d}$, where $d$ is \emph{constant} (\wrt~fixed $\HC$), and also that ... may be enumerated in $\Poly(m) = \Poly(m, \nicefrac{1}{\gamma})$ time.
We thus note that the VC case follows immediately from the general case, and now seek to prove the latter.

We now constructively show the existence of a fair-PAC-learning algorithm $\PACAlgo$ for $\HC$ and $\loss$ over domain $\X$ and codomain $\Y$.\todo{$\PACAlgo$ to $\mathcal{A}$? Macro?}

First take \emph{cover precision} $\gamma \doteq \frac{\varepsilon}{3D_{\Y}\lambda_{\loss}}$\todo{/range}.

By assumption, we may enumerate a cover $\mathcal{C}(\HC, \bm{x}, \gamma)$ in $\Poly(m, \nicefrac{1}{\gamma}) = \Poly(m, \frac{3D_{\Y}\lambda_{\loss}}{\varepsilon})$ time, which is $\Poly(m, \nicefrac{1}{\varepsilon})$, as $3D_{\Y}\lambda_{\loss}$ is constant.

The learning algorithm is thus \emph{empirical malfare minimization} over $\mathcal{C}(\HC, \bm{x}, \gamma)$.
Let
\[
\hat{h} \doteq \argmin_{h \in \mathcal{C}(\HC, \bm{x}, \gamma)} \Malfare_{p}(i \mapsto \ERisk(h; \bm{x}_i); \wv)$. \& \tilde{h} \doteq \argmin_{h \in \HC} \Malfare_{p}(i \mapsto \ERisk(h; \bm{x}_i); \wv)$. \&
\]
\todo{argmin or something that denotes breaking ties?}
\todo{x vs xi; union?}
By Lipschitz and covering properties, we thus bound the \emph{optimization error} as
\[
\Malfare_{p}(i \mapsto \ERisk(\hat{h}; \bm{x}_i); \wv) \leq \Malfare_{p}(i \mapsto \ERisk(\tilde{h}; \bm{x}_i); \wv) + \gamma D_{\Y}\lambda_{\loss} \enspace.
\]

This controls for \emph{optimization error} between true EMM solution $\tilde{h}$ and approximate EMM solution $\hat{h}$.\todo{def EMM}

We now quantify the \emph{approximation error} (due to sampling) as
\[
\argmin_{\tilde{h} \in \HC }  \Malfare()  \leq \argmin_{h^{*}} \Malfare() ? 
\]
\[
\Malfare(\tilde{h}) \leq \Malfare(\HC) + \lambda_{\loss} \left(\gamma + \sqrt{\frac{\ln \abs{\mathcal{C}(\dots)} }{2m}}\right) \leq ?
\]

Now pick $m$ as smallest $m$ s.t. $\sqrt{\dots} = \eps/3$, wh.???
$m \in \Poly(?)$.

TODO: missing tail bounds.


Dudley discretization argument (essentially Massart's lemma).

\todo{mult $n$?}

\todo{assume computability to evaluate}
\fi
%
\end{proof}

This immediately implies $\HC$ that are \emph{finite}, of bounded \emph{pseudodimension}, or bounded \emph{fat-shattering dimension} are fair-PAC-learnable. % \citep[sec 4.2]{shalev2014understanding}
For instance, this gives us \emph{classifiers} such as \emph{all possible languages} of \emph{Boolean formulae} over $d$ variables, or \emph{halfspaces} (i.e., linear hard classifiers $\HC \doteq \{ \vec{x} \mapsto \sgn(\vec{x} \cdot \vec{w}) \mid \vec{w} \in \R^{d} \}$), as well as \emph{generalized linear models}, subject to regularity constraints to appropriately control the loss function.\todo{cite GLM?}
However, it is perhaps not as powerful as it appears; it applies to \emph{fixed hypothesis classes}, thus each of the above linear models over $\R^{d}$ is fair-PAC learnable, but it says nothing about their performance as $d \to \infty$.

Note also that \cref{thm:fair-covering} leverages \emph{covering arguments} in both their \emph{statistical} and \emph{computational} capacity.
Statistical bounds based on covering are generally well-regarded, particularly when strong analytical bounds on covering numbers are available, although sharper results are possible (e.g., through the \emph{entropy integral} or majorizing measures\todo{cite}).
Furthermore, while we do construct a \emph{polynomial time} training algorithm, in many cases, optimization methods (e.g., gradient descent, Newton's method) exist to perform EMM \emph{more efficiently} and with \emph{higher accuracy}.
Worse yet, \emph{efficient enumerability} of a cover may be non-trivial in some cases;
while most covering arguments in the wild\todo{examples} are either constructive, or compositional to the point where each component can easily be constructed, it may hold for some problems that computing or enumerating a cover is computationally prohibitive\todo{coding theory cxn}.

Despite these limitations, this theorem characterizes a large class in which fair learning is tractable (both statistically and computationally).
In particular, it contains VC, bounded pseudodimension, and bounded fat-shattering dimension classes in which $\varepsilon$-ERM is efficient.\todo{citations / neural covering papers}



We now show alternative meta-conditions, which leverage convex-optimization tools to derive highly-general EMM algorithms and show fair-PAC learnability.
This is the most practical of our fair-PAC-learnability results, as the algorithm employed by the constructive proof is quite efficient, and we recommend its use in practice.
However, it is also the most restrictive, as we must assume a lot about the structure of $\HC$ to ensure efficient convex optimization.

\begin{theorem}[Fair PAC-Learning with Convex Optimization]
\todo{terminology on agnostic PAC-learnable}
Suppose $\HC$ is agnostic-PAC-learnable, and $\exists$ algorithm $\PACAlgo$ to agnostic-PAC-learn $\HC$ w.r.t.\ some loss function $\loss$, where $\PACAlgo$ simply applies a generic \emph{optimization routine} $O$ that requires only that the objective is \emph{bounded}, \emph{smooth}, and \emph{convex}.
Then $\HC$ is fair-PAC learnable \wrt{} $\loss$.

\todo{Just say exists optimizer O?}

\todo{Don't assume PAC-learnable; just assume uniformly convergent and computationally efficient?  Similar to PAC-learnable?}

\draftnote{I need to find a more precise characterization of when $\varepsilon$-optimal convex optimization is tractable.  Need also to precisely characterize that $\PACAlgo$ PAC-learns \wrt{} $\loss$.}

%
%OLD:
\if 0
Suppose $\bm{z} \in (\X \times \Y)^{m}$, and $\Risk(\bm{\theta}; \LossFunction, \bm{z})$ is \emph{bounded} and \emph{convex} in $\bm{\theta}$, and $h_{\theta}(\dots)$ may be evaluated in polynomial time (in all hyperparameters).
Suppose also the sample complexity of $\varepsilon$-$\delta$ agnostic learning $\theta^{*}$ is polynomial.
Suppose also $\Malfare(\dots)$ satisfying axioms 1-6 and \ref{def:cardinal-axioms:apd}.
Then the time and sample complexity of learning $\hat{\bm{\theta}}$ s.t.~with probability at least $1 - \delta$,
\[
\Malfare( \Risk(\hat{\bm{\theta}}; \LossFunction, \ProbDist_{1:n}); \wv ) \leq \Malfare( \Risk(\bm{\theta}^{*}; \LossFunction, \ProbDist_{1:n}); \wv ) \enspace,
\]
is polynomial in $m$, $\ln(\frac{1}{\delta})$, $\frac{1}{\varepsilon}$, and all hyperparameters.
\fi
\end{theorem}
\begin{proof}[Proof Sketch]
We show this result constructively.
By assumption, we know there exist $A, O$, such that $\PACAlgo$ PAC-learns $\HC$ by drawing a polynomially large sample $(\bm{x}, \bm{y})$, and applying $O$ to optimize
empirical risk.
%
In our construction, we instead optimize empirical malfare, and the properties of $\PACAlgo$ ensure efficient approximate optimality.
%empirical malfare.
\if 0
\[
\Risk(\dots) = ... \enspace.
\]
\todo{extend to cover optimization error?}
In particular, we define $A'$ to simply apply $O$ to the problem
\[
%O \left( \right)
\dots,
\]
which we note is \todo{assumption too weak; needs guarantee original objective is smooth and all that}.


\todo{poly increase to $\varepsilon$-learn each class}.

In particular, the sample complexity $m^{*}(A', \varepsilon, \delta)$ is $m^{*}(A', \varepsilon, \nicefrac{\delta}{n})$, \dots. \todo{Why it guarantees?  Not quite; may be unrealizable now.  Need to go back through VC / uniform learnability?} \todo{OR: mixtures? inversions?}


\fi
\end{proof}






To close this section, we now show a convenient, generic, and modular constructive characterization that yields fair-PAC-learnability for an extremely broad class of learning problem.
The constructive training algorithm is also \emph{efficient} for fixed group-count $n$, though its runtime is exponential in $n$.
This construction makes no structural assumptions about $\HC$, and assumes only that loss values of ERM solutions are \emph{stable} under small perturbations to training data %$\loss$ is Lipschitz-continuous\
(i.e., no structural assumptions, e.g., convexity on $\HC$, nor assumptions on the structure of the PAC-learning algorithm, are required).
Then if $\HC$ is PAC-learnable \wrt{} $\loss$, it is also fair-PAC-learnable.

% but does not give efficiency (can use cvx optimization for that? or covering?  State this first? or last?).  Note: lipschitz in weights space / grid / discrete covering idea VERY DIFFERENT from grid / covering HC.  VERY GENERIC: uses existing optimizer under mild conditinos on \emph{structuro of class} (not optimizer).  Similar to stability assumption.

\begin{theorem}[Fair PAC-Learning with Grid Reweighting]
\label{thm:fair-pac-stability}
Suppose loss function $\loss$ and hypothesis class $\HC$, such that for any $\bm{x} \in \X^{m}$, $\bm{x}' = \bm{x}_{1}, \dots, \bm{x}_{m}, x'$, taking ERM $\hat{h},\hat{h}'$ over $\bm{x}, \bm{x}'$, respectively, it holds that, for some \emph{stability constant} $B$ %(independent of $m$, 
we have
\[
\ERisk(\hat{h}; \bm{x}) - \ERisk(\hat{h}'; \bm{x}) \leq \mathsmaller{\frac{B}{m}} \enspace.
\]


\todo{doesn't hold; e.g., for unstable classifiers (linear regression).  Did I mean lin class?  What?}
\todo{Coro of \cref{thm:fair-pac-stability} for bounded ERM.}


\todo{I think it's wrong: need that EACH LOSS; not the risk, doesn't change much under adding points.  Should be more like
\[
\sup_{x \in \bm{x}} \abs{ \LossFunction(x, \hat{h}(x)) - \LossFunction(x, \hat{h}'(x)) } \leq \mathsmaller{\frac{B}{m}} \enspace?
\]
Think smooth loss regression, soft classification (stability).
Kind of implicitly requires unique stable soln?  Could say w.h.p.?
Cover resolution is then ?
}



%
%E.g., $\loss$ Lipschitz, $\HC$ closed under convex combination?

Then if $\HC$ is PAC-learnable \wrt{} $\loss$, then $\HC$ fair PAC-learnable \emph{for bounded $n$} \wrt{} $\loss$.
Furthermore, if $\HC$ is efficiently-PAC-learnable \wrt{} $\loss$, then $\HC$ is efficiently fair PAC-learnable \emph{for bounded $n$} \wrt{} $\loss$.
\end{theorem}
\begin{proof}[Proof Sketch]
The strategy here is to create a \emph{grid-cover} of \emph{reweightings} of the $n$ groups.
We construct a cover of reweightings of the $n$ groups, and show the $\lv$-weighted malfare is Lipschitz continuous in reweighting $\lv'$.
We then PAC-learn each reweighting, and take the empirically-malfare-minimal solution.
%and apply a generic PAC-learning algorithm to each cover-component.
%The malfare-optimal solution returned by the PAC-learners is then output, and shown to be $\epsilon$-$\delta$ optimal.


Note that the Lipschitz or stability condition $\ERisk(\hat{h}; \bm{x}) - \ERisk(\hat{h}'; \bm{x}) \leq \mathsmaller{\frac{B}{m}}$ is required to bound the size of the grid-cover; without this assumption, we can't guarantee that a finite-grid is sufficient.
%
\if 0

\todo{fixme}

[Grid construction reduction]


assume $\lambda$-Lipschitz
[remove weights by repetition approximation construction; integer ratio grid.  Grid resolution $\gamma = \frac{\varepsilon}{2\lambda}$, cover size $(\ll) (1 + \nicefrac{1}{\gamma})^{n}$ reduce to PAC with union bound, each problem $\epsilon' = \frac{\epsilon}{2}$ and $\delta' = \frac{\delta}{(cover size)}$]

note: delta problem?

\fi
%
\end{proof}

\todo{Boundedness + Nonzero Bayes-Error is sufficient: Having positive risk makes the reweighting grid behave better?}



\todo{Should we just kill grid reweighting?  Does it even work? Compare to ex 3.3 of UML?}



\if 0
{\color{blue!20!black}

Suppose $\hat{h}$ is optimal.

Problem: Pareto-optimal front; may be non-unique.
Consider $\{ (1, 0), (0, 1) \}$  Maybe works with continuity in parameter space?

Basic idea:

Take $\wv'_{i} \doteq \frac{\wv_{i} \lv^{p-1}_{i}}{\Malfare_{p-1}(\wv, \lv)}$

\[
\Malfare_{p}(\lv; \wv) 
 = \sqrt[p]{\sum_{i=1}^{n} \wv_{i} \lv^{p}_{i}}
 = \sqrt[p]{\sum_{i=1}^{n} (\wv_{i} \lv^{p-1}_{i})\lv_{i}}
 = \sqrt[\nicefrac{p}{p-1}]{\Malfare_{p-1}(\wv, \lv)} \sqrt[p]{\sum_{i=1}^{n} \frac{\wv_{i} \lv^{p-1}_{i}}{\Malfare_{p-1}(\wv, \lv)} \lv_{i}}
 = \sqrt[\nicefrac{p}{p-1}]{\Malfare_{p-1}(\wv, \lv)} \sqrt[p]{\sum_{i=1}^{n} \wv'_{i} \lv_{i}}
 = \sqrt[\nicefrac{p}{p-1}]{\Malfare_{p-1}(\wv, \lv)} \sqrt[p]{\Malfare_{1}(\wv', \lv)}
 %= \sqrt[p]{Z} \sqrt[p]{\sum_{i=1}^{n} \wv'_{i} \lv_{i}}
 %= \sqrt[p]{Z \Malfare_{1}(\lv; \wv')}
 \enspace.
\]

\todo{Iterate down to $1$?}
}
\fi




\if 0
{\color{red!40!black}%Alt thm: weighting grid search


ALT3 IDEA:

Similar to IRLS.  Do util, reweight, util, repeat ad nauseam.

Does it converge?

Start with
\[
\wv' = \wv
\]
\[
\lv \doteq \argmin_{\dots} \Mean_{1}(\lv, \wv')
\]

Then update 
\[
\wv' \propto \wv'\lv^{p-1}
\]
\[
\lv \gets \argmin_{\dots} \Mean_{1}(\lv, \wv')
\]

repeat til cvg?



property:
\[
\Mean_{p}(\lv^{(i)};\wv) \leq \Mean_{p}(\lv^{(i+1)};\wv)
\]
BC: this way the last $\Mean_{1}$ now coincides with $\Mean_{p}$

New improvement harms the weights, but helps the $\Mean_{1}$?


Not quite EM like, but close?


NOPE seems highly non-convergent.

FIX: line-search if overstep?




VISUALIZE:

Opt surface of $\Mean_{p}^{p}(\argmin_{\lv} \Mean_{1}(\lv; \wv'); \wv)$ is locally constant (where $\Mean$ is unchanged)



I think we need uniform Lipschitz (over \emph{all loss} in $\wv$, which gives us uniform over $\lv$).  This is stability.




ALT ALT IDEA:


Consider some reweighting $\wv'$.  Compute $\lv*$ at $\wv'$ and create a known value vector at $\wv'$ \todo{non-unique!  test stability by considering gradient?}.

\if 0
At  each reweighting, create a new linear (in $\wv$) upper-bound on $\Mean_{1}(\lv*; \wv)$ (i.e., $\lv^{*}$ at $\wv$)?

Need also a LB.  Can get this with Lipschitz assumption, or by cvxty / interp / contradiction; interpolating with existing known points gives lower bound, as if we did better there, then we could do better at $\wv$ too.  Interp must consider min/max over groups though.
\fi

OLD:


\todo{even if we minimize $\Mean_{1}(\lv; \wv')$, no guarantee minimum is unique?  Or is it that $Z$ is not constant?}

\todo{It's tricky.  Try cvx opt over $\wv$?  assumptions to get cvx, smooth, bounded?}

does not work; basically because the function is non-Lipschitz; so can't just grid search.


NEED ALSO: $\HC$ AND $\loss$ are Lipschitz cont?  Can close $\HC$ or $\loss \circ \HC$ under convex combination?
With this, $\lv$ becomes Lipschitz cont.
Then it goes through?  Yes, if opt not too close to 0, because $\sqrt[p]{Z}$?, $\lv$ are Lipschitz.

Note: util bounded away from 0 implies egal bound away from 0; can check first easily.

Weaker than convexity stuff (bounded cvx implies lip?)

\begin{theorem}[Fair PAC-Learning]
If PAC learnable; grid exponential in $n$ of weights; PAC learn all reweightings.

exists reweight, based on $\lv$ at (any?) optimum, s.t. $h$ is util-optimal.


small change to reweight makes small change to utilitarian-optimal, thus small change to egal-optimal.  Also everything in between?
  Lipschitz arg: pretend thing increasing has risk 0, decreasing has risk (max).  Still bounded change.



not efficient in $n$; way to make it so?


Q: what is the weighting?

\[
\Malfare_{p}(\lv; \wv) = \sqrt[p]{\sum_{i=1}^{n} \wv_{i} \lv^{p}_{i}} = \sqrt[p]{\sum_{i=1}^{n} (\wv_{i} \lv^{p-1}_{i})\lv_{i}} = \sqrt[p]{Z} \sqrt[p]{\sum_{i=1}^{n} \frac{\wv_{i} \lv^{p-1}_{i}}{Z} \lv_{i}} = \sqrt[p]{Z} \sqrt[p]{\sum_{i=1}^{n} \wv'_{i} \lv_{i}} = \sqrt[p]{Z \Malfare_{1}(\lv; \wv')}
\]
Note: Z depends on $S$!
\todo{can / 0?}
Thus
\[
\argmin \dots = \dots = \dots
\]

\[
Z = \sum_{i=1}^{n} \wv_{i} \lv^{p-1}_{i} \leq \sum_{i=1}^{n} \wv_{i} B^{p-1} \leq B^{p-1}
\]

\[
\sqrt[p]{Z} \leq B^{\nicefrac{p-1}{p}} \leq B
\]

Lipschitzness:

\[
Z = \Mean_{p-1}^{p-1}(\lv; \wv)
\]
is thus $(p-1)B \cdot L_{\lv}$ Lipschitz?
Similarly,
\[
\sqrt[p]{Z} = \sqrt{\Mean_{p-1}^{p-1}(\lv; \wv)} = \sqrt[p/p-1]{\Mean_{p-1}^{p-1}(\lv; \wv)}
\]
is thus $\dots \cdot \frac{\partial}{\partial I} \sqrt[p]{I} \leq \frac{\dots}{I}$ -Lipschitz?  I is LB on util???  Maybe not needed, since it's multiplied by $\Mean_{p}(\lv; \wv')$?

Q: how much does $\delta\wv'$ change $\lv$?  Assume can randomize cfier to get continuity?  By Jensen's, always less than linear?

NO: $\lv$ not Lipschitz in $\wv'$.  Ex: $\{h = (0, 1), h = (1, 0)\}$; discrete swap at $\wv = (.5, .5)$


What if worst group individual performance is bad?  Then $Z$ can't get too close to $0$?  Need also $Z$ Lipschitz?

\todo{Working in reverse?}

\[
\Mean_{1} = \Mean_{p}^{p}/Z?
\]

\end{theorem}
}
\fi




\todo{Add next theorem!}
\if 0
%With this limitation in mind, the next fair-PAC-learning result focuses solely on \emph{computational} aspects, implicitly assuming generalizability via standard agnostic-learning assumptions.


\begin{theorem}[Fair Agnostic PAC-Learning]
\todo{terminology on agnostic PAC-learnable}
Suppose $\HC$ is agnostic-PAC-learnable, and $\exists$ algorithm $\PACAlgo$ to agnostic-PAC-learn $\HC$, where $\PACAlgo$ simply applies a generic \emph{optimization routine} $O$ that requires only that the objective is \emph{bounded}, \emph{smooth}, and \emph{convex}.
Then $\HC$ is fair-PAC learnable \wrt{} 0-1 loss.
%
%OLD:
\if 0
Suppose $\bm{z} \in (\X \times \Y)^{m}$, and $\Risk(\bm{\theta}; \LossFunction, \bm{z})$ is \emph{bounded} and \emph{convex} in $\bm{\theta}$, and $h_{\theta}(\dots)$ may be evaluated in polynomial time (in all hyperparameters).
Suppose also the sample complexity of $\varepsilon$-$\delta$ agnostic learning $\theta^{*}$ is polynomial.
Suppose also $\Malfare(\dots)$ satisfying axioms 1-6 and \ref{def:cardinal-axioms:apd}.
Then the time and sample complexity of learning $\hat{\bm{\theta}}$ s.t.~with probability at least $1 - \delta$,
\[
\Malfare( \Risk(\hat{\bm{\theta}}; \LossFunction, \ProbDist_{1:n}); \wv ) \leq \Malfare( \Risk(\bm{\theta}^{*}; \LossFunction, \ProbDist_{1:n}); \wv ) \enspace,
\]
is polynomial in $m$, $\ln(\frac{1}{\delta})$, $\frac{1}{\varepsilon}$, and all hyperparameters.
\fi
\end{theorem}
\begin{proof}
We show this result constructively.
By assumption, we know there exist $A, O$, such that $\PACAlgo$ PAC-learns $\HC$ by drawing a polynomially large sample $(\bm{x}, \bm{y})$, and applying $O$ to optimize
\[
\Risk(\dots) = ... \enspace.
\]
\todo{extend to cover optimization error?}
In particular, we define $A'$ to simply apply $O$ to the problem
\[
%O \left( \right)
\dots,
\]
which we note is \todo{assumption too weak; needs guarantee original objective is smooth and all that}.


\todo{poly increase to $\varepsilon$-learn each class}.

In particular, the sample complexity $m^{*}(A', \varepsilon, \delta)$ is $m^{*}(A', \varepsilon, \nicefrac{\delta}{n})$, \dots. \todo{Why it guarantees?  Not quite; may be unrealizable now.  Need to go back through VC / uniform learnability?} \todo{OR: mixtures? inversions?}


\todo{Don't assume PAC-learnable; just assume uniformly convergent and computationally efficient?  Similar to PAC-learnable?}

\end{proof}

This theorem characterizes a large class in which fair learning is tractable (both statistically and computationally).
In particular, it contains VC classes in which $\varepsilon$-ERM is efficient.
We caution against blindly applying such methods in other settings, such as learning with \emph{local optimization} or \emph{proxy losses}, without carefully considering the fairness implications.
For instance it may be the case that training an SVM with \emph{hinge loss} as a proxy for \emph{ramp loss} or \emph{0-1 loss} results in a few high-hinge-loss outliers for group $\PACAlgo$, thus unfairly incentivizing better treatment of group $\PACAlgo$, at the cost of performance for group $B$.
Similarly, optimizing a neural network may quickly converge to a \emph{locally optimal} solution that favors some \emph{easily mutually satisfied} subset of groups, and thus may %(unfairly
terminate before identifying a solution that works for all groups. %, a local optimum that is effective for some groups not others and without matching lower bounds it is difficult to automatically detect this situation

\fi


\paragraph{Nonlearnability and a warning in closing}
We caution against blindly applying such methods in other settings without learnability guarantees, such as learning with \emph{local optimization} or \emph{proxy losses}, without carefully considering the fairness implications.
For instance it may be the case that training an SVM with \emph{hinge loss} as a proxy for \emph{ramp loss} or \emph{0-1 loss} results in a few high-hinge-loss outliers for group $\PACAlgo$, thus \emph{unfairly} incentivizing better treatment of group $\PACAlgo$, at the cost of performance for group $B$.
Similarly, optimizing a neural network may converge to a \emph{locally optimal} solution that favors some \emph{easily mutually satisfied} subset of groups, and thus may %(unfairly)
terminate before identifying a solution that works for all groups.
In this sense, without learnability guarantees, we are unable to ensure fairness, making similar claims of fairness in these settings naively optimistic at best, and shallow platitudes at worst.



==> paper/pac2.tex <==


NOTE: THIS DOCUMENT USES A STRONGER PAC CONCEPT (POLYNOMIAL)

\todo{Check cvx concave proofs}


\section{Fair PAC-Learning II}
\label{sec:pac}

The remainder of this document builds upon and refines the ideas of \cref{sec:est-learn:pac}.
Some definitions are modified.
Whereas \cref{sec:est-learn:pac} is primarily concerned with constructing fair-PAC learners, the idea here is primarily to relate PAC and fair-PAC learning, with the understanding that this allows the vast breadth of research of PAC-learning algorithms and necessary / sufficient conditions to be applied to fair-PAC learning.
In particular, we show a hierarchy of fair-learnability via generic statistical and computational learning theoretic bounds and reductions.


\subsection{Some Definitions}

\paragraph{A Quick Recap}
We define the \emph{risk} of hypothesis $h: \X \to \Y$ \wrt{} loss $\LossFunction: \Y \times \Y \to \R_{+}$ on distribution $\ProbDist$ over $(\X \times \Y)$ as
\[
\Risk(h; \LossFunction, \ProbDist) \doteq \Expect_{(x, y) \distributed \ProbDist} \bigl[ \loss(y, h(x)) \bigr] \enspace,
\]
and the empirical risk on sample $\bm{z} \in (\X \times \Y)^{m}$ as
\[
\ERisk(h; \LossFunction, \bm{z}) \doteq \EExpect_{(x, y) \in \bm{z}} \bigl[ \LossFunction(y, h(x)) \bigr] \enspace.
\]
\todo{Resolve $\LossFunction \loss$ redundancy.}
\todo{Ground truth / prediction spaces may differ.}

We reiterate that the \emph{$p$-power mean Malfare} on sentiment (loss) vector $\lv$ with weighting $\wv$ is
\[
\Malfare_{p}(\lv; \wv) \doteq
  \begin{cases}
  p \in \R \setminus \{0\} & \displaystyle \sqrt[p]{\int_{\wv} \lv^{p}(\omega) \, \mathrm{d}(\omega) } = \sqrt[p]{\Expect_{\omega \distributed \wv}[\lv^{p}(\omega)]} \\
  p = -\infty & \displaystyle \min_{\omega \in \Support(\wv)} \lv(\omega) \\
  p = 0 & \displaystyle \exp\left( \int_{\wv} \ln \lv(\omega) \, \mathrm{d}(\omega) \right) = \exp\left( \Expect_{\omega \distributed \wv}[\ln \lv(\omega)] \right) \\
  p = \infty & \displaystyle \max_{\omega \in \Support(\wv)} \lv(\omega) \\
  \end{cases}
  \enspace,
\]
where here we are concerned only with $p \geq 1$,
Finally the \emph{empirical malfare minimization} (EMM) principle generalizes ERM to compute
\[
\argmin_{h \in \HC} \hat{\Malfare}(h; \bm{z}_{1:n}, \Utility) = \argmin_{h \in \HC} \Malfare\left(i \mapsto \ERisk(h; \LossFunction, \bm{z}_{i}); \wv \right) \enspace.
%\EExpect_{(x, y) \in \bm{z}_{i}}[\LossFunction(y, h(x))]
\]

\paragraph{Hypothesis Classes and Sequences}

We now define \emph{hypothesis class sequences}, required to discuss nontrivial \emph{computational complexity} in learning.
This definition is adapted from \citep[Def.~8.1]{shalev2014understanding}, which treats only \emph{binary classification}.


%\todo{Swap to sequences; note generalize to real or vector-valued parameter.}
\begin{definition}[Hypothesis Class Sequence]
A \emph{hypothesis class sequence} $\HC = (\HC_{1}, \HC_{2}, \dots)$ is a \emph{nested sequence} of \emph{hypothesis classes} mapping $\X \to \Y$. %, indexed by $\N$ or $\R$.
In other words, $\HC_{1} \subseteq \HC_{2} \subseteq \dots$. % \subseteq (\X \to \Y)$.

\draftnote{Should we have domains $\X_{1}, \X_{2}, \dots$?}


%\todo{Good name: mata-class is confusing, class sequence is confusing.}
\end{definition}

Usually, %$(i \leq j) \implies (\HC_{i} \subseteq \HC_{j})$, and 
$\HC_{i}$ is easily derived from $\HC_{j}$.\todo{Make this part of def}
For instance, \emph{linear classifiers} naturally form a sequence of families using their \emph{dimension}:
\[
\HC_{\DSeq} \doteq \left\{ \vec{x} \mapsto \sgn\bigl(\vec{x} \cdot (\vec{w} \circ \vec{0}) \bigr) \, \middle | \, \vec{w} \in \R^{\DSeq} \right\} \enspace.
\]
Here each $\HC_{i}$ is defined over domain $\R^{\infty}$, but it is more natural to discuss them as objects over $\R^{\DSeq}$.

Similarly, \emph{%unit-scale 
univariate polynomial regression} naturally decomposes as
\[
\HC_{\DSeq} \doteq \left\{ x \mapsto (x, x^{2}, \dots, x^{\DSeq}) \cdot \vec{w} \, \middle | \, \vec{w} \in [0, 1]^{\DSeq} \right\} \enspace.
\]

There is no special reason for $\HC$ to be a \emph{sequence}; \emph{fractional} $\DSeq$ are quite natural when $\HC_{\DSeq}$ is defined by a real-valued \emph{regularity constraint}, and more generally, a POSET of classes (comparisons defined by containment) arises naturally given \emph{multiple complexity parameters}, e.g., \emph{depth $D$ neural networks} with \emph{layer widths} vector $\vec{W}$, or \emph{multivariate polynomial regression}.

This concept is necessary, because showing computational-hardness of a statistically-easy learning problem essentially boils down to selecting a hypothesis class sequence such that learning \emph{time complexity} grows \emph{superpolynomially faster} (in $\DSeq$) than learning \emph{sample complexity}.

\if 0 %TODO
\begin{observation}

\todo{We make no mention of \emph{boundedness} of $\HC$ ...}

\todo{Boundedness comment, loss function and/or domain control it.}


\todo{Problem: need to parameterize $\X$ too (projections maybe), otherwise data size can be infinite and need to worry about representation too much?}
\end{observation}
\fi



For context, we first present a generalized notion of PAC-learnability, which we then generalize to fair-PAC-learnability.
Standard presentations consider only classification under 0-1 loss, but some authors consider generalized notions for other learning problems (see, e.g., \citet[Definition~3.4]{shalev2014understanding}).


\todo{Check against 3.4 of UML! Classification is \citet[Definition~3.1]{shalev2014understanding}.  Note: they don't assume polynomial!  Is it the same?}
\begin{definition}[PAC-Learnability]
\label{def:pac}
%An algorithm $\PACAlgo$ is said to be 
Suppose \emph{nested hypothesis class sequence} $\HC_{1} \subseteq \HC_{2} \subseteq \dots$, % \subseteq \X \to \Y$
all over $\X \to \Y$, and \emph{loss function} $\ell: \Y \times \Y \to \R_{0+}$.\cyrus{Often target space and codomain don't match: interval estimators, recommender systems, and density estimators.}
We say $\HC$ is \emph{PAC-learnable} \wrt{} $\ell$ if $\exists$ a (randomized) algorithm $\PACAlgo$, such that $\forall$:
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item sequence index $\DSeq$;
\item instance distribution $\ProbDist$ over $\X \times \Y$;
\item additive approximation error $\varepsilon > 0$;
\item failure probability $\delta \in (0, 1)$;
\end{enumerate}
it holds that $\PACAlgo$ can identify a hypothesis $\hat{h} \in \HC$, i.e., $\hat{h} \gets \PACAlgo(p, \wv, \ProbDist_{1:\NGroups}, \varepsilon, \delta, \DSeq)$, such that\todo{Call it $\PACAlgo_{\HC}$?}
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\PACAlgo$ has $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, \DSeq)$ expected sample complexity; and \cyrus{Polynomial or finite?  Not quite the same in general?}\cyrus{Write as finite.}
%\emph{polynomial} (in $\NGroups$, $\nicefrac{1}{\varepsilon}$, and $\nicefrac{1}{\delta}$) expected time complexity.%, space, entropy, and sample complexity (i.e., requires polynomially bounded computational, memory, randomness, and training instances);
\item with probability at least $1 - \delta$ (over randomness of $\PACAlgo$), $\hat{h}$ obeys
\[
%\Expect_{(x, y) \distributed \ProbDist} \bigl[ \loss(y, \hat{h}(x)) \bigr] \leq \inf_{h^{*} \in \HC} \Expect_{(x, y) \distributed \ProbDist} \bigl[\loss(y, h^{*}(x)) \bigr] + \varepsilon \enspace.
\Risk(\smash{\hat{h}}; \LossFunction, \ProbDist) \leq \inf_{h^{*} \in \HC} \Risk(h^{*}; \LossFunction, \ProbDist) + \varepsilon \enspace.
\]
\todo{$\hat{h}$ is \emph{measurable}?}\todo{Check remark 3.1 of UML}
\end{enumerate}
The class of such learning problems is denoted $\PAC$, thus we write $(\HC, \LossFunction) \in \PAC$ to denote PAC-learnability.

\medskip

Additionally, $\HC$ is \emph{polynomial-time-PAC-learnable} if %$\PACAlgo$
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\setcounter{enumi}{3}
\item $\PACAlgo$ runs in $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, \DSeq)$ expected time complexity;
\item the output of $\PACAlgo$ is sufficient to evaluate $\hat{h}(\cdot)$ in $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, \DSeq)$ expected time complexity.
\end{enumerate}
The subclass of polynomial-time learning problems is denoted $\PAC_{\Poly}$, thus we write $(\HC, \LossFunction) \in \PAC_{\Poly}$ to denote poly-time PAC-learnability.

\medskip

Finally, if $\ProbDist$ is restricted such that
\[
\exists h \in \HC_{\DSeq} \text{ s.t.\ } \Risk(h; \LossFunction, \ProbDist) = 0 \enspace,
\]
then $(\HC, \LossFunction)$ is \emph{realizable-PAC-learnable}, written $(\HC, \LossFunction) \in \PAC^{\Realizable}$. %, otherwise (in general) $(\HC, \LossFunction)$ is \emph{agnostic PAC learnable}, written $(\HC, \LossFunction) \in \PAC^{\Agnostic}$.
\end{definition}

\todo{Add this observation in better form:}
\if 0
\begin{observation}
It is clear from the definition that

\[
\PAC(\LossFunction) \subseteq \PAC^{\Realizable}(\LossFunction)
\]

\[
\PAC_{\Poly}(\LossFunction) \subseteq \PAC_{\Poly}^{\Realizable}(\LossFunction)
\]

\[
\PAC_{\Poly}(\LossFunction) \subseteq \PAC(\LossFunction)
\]

\[
\PAC_{\Poly}^{\Realizable}(\LossFunction) \subseteq \PAC^{\Realizable}(\LossFunction)
\]
\end{observation}
\fi

\todo{
TODO: NOTE ON WHY SEQS; GENERALIZE TO DAG; subjectivity of seq.}

\todo{
note taking all $\HC_{i} = \dots $, or even $\lim_{i \to \infty} \HC_{i} \setminus \HC_{i-1} = \emptyset$, then ignore sequence.
}

\begin{observation}[On Realizable Learning]
Our definition of realizability appears to differ from the standard form, in which $\ProbDist$ is a distribution over only $\X$, and $y$ is simply computed as $h^{*}(x)$, for some $h^{*} \in \HC$.
We instead constrain $\ProbDist$ such that there exists a 0-risk $h^{*} \in \HC$, which is equivalent for any loss function $\LossFunction$ such that $\LossFunction(y, \hat{y}) = 0 \Leftrightarrow y = \hat{y}$, e.g., 0-1 classification loss, absolute or square regression loss.
With our definition, it is much clearer that realizable learning is a special case of agnostic learning,
%is that the connection to agnostic learning is much clearer and furthermore the generalization to fair learning is also more straightforward. And maybe not really that last part.
and furthermore, we handle a much broader class of problems, for which there may be some amount of \emph{noise}, or wherein a ground truth may not even exist.

For instance, in a \emph{recommender system}, $y$ may represent the \emph{set of items} that $x$ will like, and $h$ may predict a singleton set, and thus we take $\LossFunction(y, \{\hat{y}\}) = \1_{y}(\hat{y})$.
There is no ground-truth here, but rather we seek a \emph{compatible solution} that recommends appropriate items to everyone.

Similarly, in high-dimensional classification, we often treat classifier output as a \emph{ranked list} of predictions, and the \emph{top-$k$ loss} is taken to be $\LossFunction(y, \hat{y}) = \1_{\hat{y}_{1:k}}(y)$.
Again, no ground truth exists, but 0-risk learning is still possible if there is not ``too much'' ambiguity (i.e., foxes and dogs can be confused, as long as they are separated from horses and zebras).

 %In particular a top K classifier predicts an ordered list of class estimates in order of likelihood and incurs 0 loss if the true class is within the top K predicted classes. For ambiguous examples we may remain the allies obal so long as no example is to ambiguous for instance a dog and a Fox might be ambiguous as long as they can clearly be distinguished from a horse.

Finally, the task of an \emph{interval estimator} is to predict an \emph{interval} for every $x$ in which $y$ must lie, thus again $\LossFunction(y, \hat{y}) = \1_{\hat{y}}(y)$.
Under bounded noise conditions, the \emph{interval estimation} problem can easily be realizable, even if it is impossible to exactly recover the \emph{ground truth} from noisy labels.

\if 0
\todo{xplain}

text description
recommender system
interval estimator

no ground truth?
\fi
\end{observation}

\todo{Why we need d seq: must assume X is finite (discretized), eventually dist starts to repeat, then it becomes weighted learning problem?}

\todo{Assume $P \neq NP$ somewhere.}

We now generalize this concept to \emph{fair-PAC-learnability}.
In particular, we replace the \emph{univariate risk-minimization} task with a \emph{multivariate malfare-minimization} task.
Following the theory of \cref{sec:pop-mean:prop}, we do not commit to any particular objective, but instead require that a fair-PAC-learner is able to maximize \emph{any} fair malfare function satisfying the standard axioms.
Furthermore, here problem instances grow not just in problem complexity $\DSeq$, but also in the number of groups $\NGroups$.
%We allow sampling from the \emph{joint distribution} of \emph{per-group} instances, thus sample complexity requirements remains unchanged, but computational complexity may now depend $\NGroups$.

\begin{definition}[Fair Agnostic PAC-Learnability]
\label{def:fair-pac}
%An algorithm $\PACAlgo$ is said to be 
Suppose \emph{nested hypothesis class sequence} $\HC_{1} \subseteq \HC_{2} \subseteq \dots \subseteq \X \to \Y$, and \emph{loss function} $\ell: \Y \times \Y \to \R_{0+}$.
We say $\HC$ is \emph{fair PAC-learnable} \wrt{} \emph{group count} $\NGroups$ and \emph{loss function} $\ell$ if $\exists$ a (randomized) algorithm $\PACAlgo$, such that $\forall$:
\todo{poly computable}
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item sequence index $\DSeq$;
\item group count $\NGroups$;
\item instance distribution $\ProbDist_{1:n}$ over $(\X \times \Y)^{n}$;
\item group weights measure $\wv$ over $\{1, \dots, n\}$;
\item malfare concept $\Malfare(\dots)$ satisfying axioms 1-7 and \ref{def:cardinal-axioms:apd};\todo{macro for axioms.}
\if 0
\draftnote{%I.e., 
Equivalently, $\Malfare(\dots)$ is %necessarily 
some convex power mean $\Malfare_{p}(\dots)$, thus $p \geq 1$.}
\fi
\item additive approximation error $\varepsilon > 0$;
\item failure probability $\delta \in (0, 1)$;
\end{enumerate}
it holds that $\PACAlgo$ can identify a hypothesis $\hat{h} \in \HC$ such that
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\PACAlgo$ has $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, \DSeq)$ expected sample complexity; and\todo{Do I want $\NGroups$ in the poly?  Or not needed?  Prove it either way?} %\emph{polynomial} (in $\nicefrac{1}{\varepsilon}$, and $\nicefrac{1}{\delta}$) expected time complexity.%, space, entropy, and sample complexity (i.e., requires polynomially bounded computational, memory, randomness, and training instances);
\item with probability at least $1 - \delta$ (over randomness of $\PACAlgo$), $\hat{h}$ obeys
\[
%\Malfare\left(i \mapsto \biggl( \Expect_{(x, y) \distributed \ProbDist_{i}} \bigl[ \loss(y, \hat{h}(x)) \bigr] \biggr); \wv \right) \leq \argmin_{h \in \HC} \Malfare \left(i \mapsto \biggl(\Expect_{(x, y) \distributed \ProbDist_{i}} \bigl[\loss(y, h(x)) \bigr] \biggr); \wv \right) + \varepsilon \enspace.
\Malfare\left(i \mapsto \Risk(\smash{\hat{h}}; \LossFunction, \ProbDist_{i}); \wv \right) \leq \argmin_{h^{*} \in \HC} \Malfare \left(i \mapsto \Risk(h^{*}; \LossFunction, \ProbDist_{i}); \wv \right) + \varepsilon \enspace.
\]
%
\todo{$\hat{h}$ is \emph{measurable}?}
\end{enumerate}

The class of such fair learning problems is denoted $\FPAC$, thus we write $(\HC, \LossFunction) \in \FPAC$ to denote fair-PAC-learnability.

\medskip

Additionally, $\HC$ is \emph{polynomial-time-fair-PAC-learnable} if %$\PACAlgo$
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\setcounter{enumi}{3}
\item $\PACAlgo$ runs in $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, \DSeq, \NGroups)$ expected time complexity;
\item the output of $\PACAlgo$ is sufficient to evaluate $\hat{h}(\cdot)$ in $\Poly(\nicefrac{1}{\varepsilon}, \nicefrac{1}{\delta}, \DSeq)$ expected time complexity.\todo{Do I need / want $\NGroups$ as part of the evaluation TC?}
\end{enumerate}

The subclass of polynomial-time fair learning problems is denoted $\FPAC_{\Poly}$, thus we write $(\HC, \LossFunction) \in \FPAC_{\Poly}$ to denote poly-time fair-PAC-learnability.

\medskip

Finally, if $\ProbDist$ is restricted such that
\[
\exists h \in \HC_{\DSeq} \text{ s.t.\ } \sup_{i \in 1, \dots, n} \Risk(h; \LossFunction, \ProbDist_{i}) = 0 \enspace,
\todo{Could rewrite as $\Malfare_{\infty}$ condition?}
\]
then $(\HC, \LossFunction)$ is \emph{realizable-fair-PAC-learnable}, written $(\HC, \LossFunction) \in \FPAC^{\Realizable}$.
%
\end{definition}


\draftnote{Should these be expected or worst-case complexities?}

\begin{observation}

$\Malfare$ is $\Malfare_{p}$ for $p \in [1, \infty)$

Taking $\NGroups=1$ implies $\bm{w} = (1)$ and $\Malfare_{p}(\lv; \wv) = \lv_{1}$, thus reducing the problem to standard PAC-learning.\todo{Agnostic / realizable assumption too}


\end{observation}






\paragraph{An aside on the flexibility of fair-PAC-learnability}

Note that the generalized definition of (fair) PAC-learnability is sufficiently broad so as to include many \emph{supervised}, \emph{semi-supervised}, and \emph{unsupervised} learning problems.

While this is not immediately apparent, consider that, for instance, %learning a 
\emph{$k$-means clustering} can be expressed as a \emph{learning problem} where the task is to identify a set of $k$ vectors in $\R^{\DSeq}$ where the hypothesis class maps a vector $\vec{x}$ on to the nearest cluster center, and the loss function is the square distance.\todo{Convert to computational hardness reduction?} 
%
This is %actually 
a surprisingly natural fairness issue %; for instance clustering is somewhat related to computing a Steiner tree Which 
when cast as a \emph{resource allocation problem};
if, for instance each cluster center represents a cellphone tower, %it is then a fairness issue 
then we seek to place towers to serve \emph{all groups}, and to avoid serving one or more groups at the expense of others. %one group well while neglecting others.


\todo{ALSO MEAN ESTIMATION; PARAMETRIC (AND NONPARAM) DISTRIBUTION ESTIMATION (see uml 13.7 exercise 2).}

\todo{Active and online settings.}



\todo{Contrast with cell donian learner. Mind paragraph sent to Michael. 7 things this intro}





\todo{Restore figure?}
\if 0
\subsection{OLD FIGURE}

TODO: GENERALIZE SPLIT SUBGROUP:

weakly or $\Malfare$-PAC learnable: specific function (e.g., minimize -egal), relax cdtns.

strongly FAIR-PL: poly in $\NGroups$, properties of $\HC$, or properties / classes of loss?

generalize m-estimator

realizable / agnostic.

data / dist dependent.

statistical: glivenko-cantelli / donsker

efficient: time poly.

\begin{figure}
\begin{tikzpicture}[
    scale=3,
    axs/.style={rectangle,draw,thick,rounded corners=0.5ex,fill=blue!10!white},
    props/.style={rectangle,draw,thick,rounded corners=0.5ex,fill=red!10!white},
    arrs/.style={line width=0.5mm, -{Stealth[length=4mm, open]}},
  ]

\node[axs] (a1) at (-1, -1) {PAC-Learnable};
\node[axs] (a1) at (-1, 0) {Realizable};
\node[axs] (a1) at (-1, 1) {Agnostic};


\node[axs] (a1) at (0, -1) {Sample-Efficient};
\node[axs] (a1) at (1, -1) {Computation-Efficient};

\end{tikzpicture}

Each quadrant has subclasses:

$n=1$: full
strong: poly in $\NGroups$ / other params of $\HC$
uniform over $\loss$ family


\end{figure}
\fi

\todo{Reweighting classes}


\todo{Antithm: reweighting.}

\todo{Non-reduction: minimax or discrete optimization? submodularity? Want PAC $\not \implies$ Fair PAC}

\todo{Can weighting just be factored into the loss?  Don't think so.}


%\subsection{Result 0: Trivialities}

\paragraph{Some trivial reductions}

\if 0
\begin{observation}[Group Count Hierarchy]
$\NGroups$ fair-PAC implies $\NGroups' \leq \NGroups$ fair-PAC. 
\end{observation}
\todo{describe / write.}
\fi

\begin{observation}
\label{obs:pac2fpac}
\[
(\HC, \LossFunction) \in \FPAC^{y}_{x} \implies(\HC, \LossFunction) \in \PAC^{y}_{x} \enspace,
\]
where $x$ denotes either poly-time or unconstrained, and $y$ denotes either realizable or agnostic.
%(Efficient) fair-PAC $\implies$ (efficient) PAC.
\end{observation}
We first observe (immediately from \cref{def:pac,def:fair-pac}) that PAC-learning is a special case of fair-PAC-learning.
In particular, taking $\NGroups=1$ implies $\Mean_{p}(\lv) = \Mean_{1}(\lv) = \lv_{1}$, thus \emph{malfare-minimization} coincides with \emph{risk minimization}.
%This is because all power means coincide with the identity function in this case thus it reduces to a risk bound.
The more interesting question, which we seek to answer in the remainder of this document, is \emph{when} and \emph{whether} the \emph{converse} holds.
In particular, when possible, we would like to show practical, sample-and-compute-efficient \emph{constructive reductions}.

\begin{observation}[Agnosticism and Realizability]
$(\HC, \LossFunction) \in \FPAC_{\Poly} \implies(\HC, \LossFunction) \in \FPAC_{\Poly}^{\Realizable}$.

\todo{Explain notation}

\end{observation}


\subsection{Characterizing Fair Statistical Learnability}
\label{sec:ftfsl}


We first consider only questions of \emph{statistical learning}.
In other words, we ignore computation for now, and show only that \emph{there exist} fair-PAC-learning algorithms of unbounded runtime.
In particular, we show a generalization of the \emph{fundamental theorem of statistical learning} to fair learning problems.
The aforementioned result relates \emph{uniform convergence} and \emph{PAC-learnability}, and is generally stated for binary classification only.
We define a natural generalization of uniform convergence to arbitrary learning problems within our framework, and then show conditions under which a generalized fundamental theorem of (fair) statistical learning holds.
In particular, we show that, neglecting computational concerns, PAC-learnability and fair-PAC learnability are equivalent.

\draftnote{
Here we find that for many learning problems, the conditions for fair PAC-learnability are identical to those for PAC-learnability.
We will find that under realizability, the same equivalence holds, however we conjecture that in general, agnostic fair PAC-learning and agnostic PAC-learning are not poly-time equivalent.}


\todo{Note: nothing fairness related here; it applies though}

We first define a \emph{generalized notion} of \emph{uniform convergence} as defined by \citep{shalev2014understanding}\todo{ref}.
In particular, our definition applies to \emph{any bounded loss function},\footnote{Boundedness should not be strictly necessary for learnability even uniform convergence, but vastly simplifies all aspects of the analysis.  In many cases, it can be relaxed to moment-conditions, such as \emph{sub-Gaussian} or \emph{sub-exponential} assumptions.} thus greatly generalizes the standard notion for binary classification.

\begin{definition}[Uniform Convergence]
\label{def:uc}
Suppose $\LossFunction: \Y \times \Y \to [0, \frange] \subseteq \R$ and hypothesis class $\HC \subseteq \X \to \Y$.\todo{Is boundedness needed?}
Let $\F \doteq \LossFunction \circ \HC$.
We say $(\HC, \LossFunction) \in \UC$ or $\F \in \UC$ if
\[
\lim_{m \to \infty} \sup_{\ProbDist} \Expect_{\bm{x} \distributed \ProbDist^{m}}\left[ \sup_{h \in \HC} \abs{ \ERisk(h; \LossFunction, \bm{x}) - \Risk(h; \LossFunction, \ProbDist) } \right] = 0 \enspace.
\]

%\todo{Under boundedness: equivalent? to:}

\end{definition}
\begin{observation}
We stress that this definition is both uniform over the \emph{function family} $\F$ and uniform over \emph{all possible distributions} $\ProbDist$.
The standard definition of \emph{uniform convergence in probability} applies to a singular $\ProbDist$, however it is standard in PAC-learning and VC theory to assume uniformity over $\ProbDist$, so we adopt this convention.

%Our definition generalizes 
Standard uniform convergence definitions consider only the convergence of \emph{empirical frequencies} of events to their \emph{true frequencies}, whereas we generalize to consider uniform convergence of the \emph{empirical means of functions} to their \emph{expected values}.
\end{observation}



%Polynomial rate:
\if 0
\begin{definition}[Polynomial-Rate Uniform Convergence]
\label{def:uc-poly}
Suppose as in \cref{def:uc}.
We say $(\HC, \LossFunction)$ or $\F$ has \emph{polynomial-rate uniform convergence}, written $(\HC, \LossFunction) \in \UC_{\Poly}$ or $\F \in \UC_{\Poly}$, if\todo{Nested seqs?  Changing $\X$?}
\[
%\lim_{m \to \infty}
\sup_{\ProbDist} \Expect_{\bm{x} \distributed \ProbDist^{m}}\left[ \sup_{h \in \HC} \abs{ \ERisk(h; \LossFunction, \bm{x}) - \Risk(h; \LossFunction, \ProbDist) } \right] \in \LandauO \frac{1}{\Poly(m)} %\LandauO \Poly \frac{1}{m} \enspace.
\]

NEED M POLY IN 1/EPSILON

TODO: none of this.

\[
m^{*}(\frac{1}{\varepsilon}) = \inf \left( m :  \sup_{\ProbDist} \Expect_{\bm{x} \distributed \ProbDist^{m}}\left[ \sup_{h \in \HC} \abs{ \ERisk(h; \LossFunction, \bm{x}) - \Risk(h; \LossFunction, \ProbDist) } \right] \leq \varepsilon \right) = \inf(m : SD(m) \leq \varepsilon) = SD^{-1}(\varepsilon)
\]

So we need
\[
SD^{-1}(\varepsilon) \in \Poly(\frac{1}{\varepsilon})
\]


\[
SD^{-1}(\Poly^{-1}(\varepsilon)) \in \frac{1}{\varepsilon}
\]
which implies
\[
SD( ... )
\]

I'm not sure.  I guess we just want polynomial sample complexity?



\end{definition}


TODO: simple UC / PAC (ignore efficiency).



\begin{property}[Establishing the Uniform Convergence Hierarchy]
$(\HC, \LossFunction) \in \UC_{\Poly} \implies (\HC, \LossFunction) \in \UC$, but
there exist $(\HC, \LossFunction)$ such that the converse is false.

In particular, for any infinite $\X$, $\Y = [0, 1]$, and regression loss function of the form $\LossFunction(y, \hat{y})$ such that $\LossFunction(y, \hat{y}) = 0 \Leftrightarrow y = \hat{y}$, there exist $\HC \subseteq \X \to [0, 1]$ that are only superpolynomially-rate uniformly convergent. % $ = Q(y - \hat{y})$, %where $Q(0) = 0$ uniquely minimizes $Q$ is such a case.
\end{property}
\begin{proof}

Suppose hypothesis class sequence $\HC$ mapping $\X \to \{0, 1\}$, such that for all $k \in \N$, $\VC(\HC_{i})$ is finite.  %$i \mapsto \VC(\HC_{i}) \in \LandauOmega(i^k)$ (i.e., the VC dimension grows superpolynomially).
Now define the \emph{regression hypothesis class}
\[
\HC_{\R} \doteq \{ x \mapsto \sum_{i=0}^{\infty} 2^{-1} h_i(x) | h_i \in \HC_{i} \} \enspace,
\]
and note that $\HC_{\R} \subseteq \X \to [0, 1]$.
In other words, in binary representation, a hypothesis $h \in \HC_{\R}$ takes hypotheses $h_{1:\infty} \in \HC_{1:\infty}$, and combines them as
\[
h(x) = 0 \, . \, h_{1}(x) \, h_{2}(x) \, h_{3}(x) \, \dots \enspace.
\]

%Furthermore, worst-casing over $\ProbDist$, we may select each $\HC_{i}$ to be \emph{orthogonal} to all $\HC_{j}$, in the sense that ...
\draftnote{Somehow need $\HC_{i}$ to be orthogonal to $\HC_{j}$, maybe want $\X = \X_{1}, \X_{2}, \dots$, and take
\[
\HC_{\R} \doteq \{ x \mapsto \sum_{i=0}^{\infty} 2^{-1} h_i(x_i) | h_i \in \HC_{i} \} \enspace?
\]
}

Now, note that for every $\varepsilon > 0$, there exists some $i(\varepsilon) \in \N$, $\gamma(\varepsilon) > 0$, which mutually depend on $\LossFunction$ (existence guaranteed by the assumption $y \neq \hat{y} \implies \LossFunction(y, \hat{y}) > 0$), such that for some possible distributions, a $\gamma$-uniform estimate of $\HC_{i(\varepsilon)}$ is \emph{required} to uniformly estimate $\HC_{\R}$.
Because $i(\varepsilon)$, $\gamma$ may be taken worst-case over distributions, they depend only on $\LossFunction$.

We now may select each $\HC_{i(\varepsilon)}$ such that $\VC(\HC_{i(\varepsilon)})$ grows sufficiently rapidly in $\varepsilon$ such that an arbitrary sample complexity lower bound $m_{\downarrow}(\frac{1}{\varepsilon})$ is required to learn $\HC_{i(\varepsilon)}$, and thus $\HC_{\R}$.
In particular, taking $\HC_{i(\varepsilon)} \in \gamma(\varepsilon)\exp(\Omega \frac{1}{\varepsilon}))$, and applying the standard realizable sample-complexity lower-bound, we have 
\[
m_{\downarrow}(\frac{1}{\varepsilon}) \mapsto \LandauOmega \frac{\VC(\HC_{i(\varepsilon)})}{\gamma(\varepsilon)} = \exp \Omega \frac{1}{\varepsilon} \enspace.
\]

We may thus conclude that $\HC$ may be selected such that uniform convergence in $\Poly(\frac{1}{\varepsilon})$ samples is impossible.
Indeed, we have shown that there exist $\HC$ for which exponential sample complexity is necessary, and by this method may create an arbitrarily large necessarily sample complexity.
Note also that since each $\VC(\HC_{i})$ is finite, the class is uniformly convergent, thus we have $(\HC, \LossFunction) \in \UC$ and $(\HC, \LossFunction) \not\in \UC_{\Poly}$.

\draftnote{I think I actually need to assume $\LossFunction(y, \hat{y}) \leq C\abs{y - \hat{y}}$ to show it's uniformly convergent.}

\todo{Prove it's UC} 
%which quantifies how rapidly $\VC(\HC_{i(\varepsilon)})$ must grow to ensure a superpolynomial (or arbitrarily large) sample complexity for learning $(\HC_{\R}, \LossFunction)$.
%
%We now simply take $\HC_{i}$ such that $\VC(\HC_{i(\varepsilon)})$ increases sufficiently rapidly so as to ensure a superpolynomial (in $\frac{1}{\varepsilon})$ sample-complexity lower bound.
%
%(in the realizable case) is \emph{required} to  
%
% both of which may be bounded via $Q$ 
%
\if 0
Under any $\LossFunction$ such that $\LossFunction(y, \hat{y}) = 0$ iff $y = \hat{y}$, and $\LossFunction(a, a \pm \varepsilon)$ approaches $0$ ``sufficiently slowly''\draftnote{I need to characterize this, but any $\abs{y - \hat{y}}^{p}$ should be fine.}

$\HC_{R}$ is uniformly learnable, but with superpolynomial sample complexity.


Intuitively, each $\HC_{i}$ independently learns a single bit of the prediction.


Problem: have $0.x1\bar{0} = 0.x0\bar{1}$.
Fix: work in quaternary?  I.e., assume that in true soln, all odd bits are 0?  Or $\HC$ can enforce that?
Then firsst mistake at bit $2i$ means loss $\geq q(2^{-2i} - (2^{-2i+1} + \dots)) = \frac{1}{3 \cdot 2^{2i}}$?

If 1 to 0 mistake:
\[
\LossFunction(y, y_{1:2i} + \frac{1}{3 \cdot 2^{2i}}) \leq \LossFunction(y, \hat{y}) \leq \LossFunction(y, y_{1:2i})
\]
If 0 to 1 mistake:
?
\fi
%
\end{proof}

\draftnote{Conjecture: $\displaystyle\F \in \UC_{\Poly} \Leftrightarrow \sup_{\ProbDist} \mathcal{N}(\F, \ell_{2}(\ProbDist,%^{m}, 
\varepsilon)) \in \Poly(\varepsilon)$}

\todo{C \& C}
\if 0
\begin{property}[Convergence and Covering]

\[
\sup_{\varepsilon > 0} \frac{\varepsilon}{2} \sqrt{\ln \mathcal{N}(\varepsilon, \F, \ell_{2}(\ProbDist))} \leq_{L} \mathcal{G}_{m}(\F, \ProbDist) \leq_{L} \int_{0}^{\infty} \sqrt{\ln \mathcal{N}(\varepsilon, \F, \ell_{2}(\ProbDist))} \, \mathrm{d}\varepsilon \enspace.
\]

\todo{Missing $m$ normalization!}


So if we assume PUC, then we have
\[
\mathcal{G}_{m}(\F, \ProbDist) \leq \ln(m) SD %\frac{}{\varepsilon^{2}}
\]

Now, we set SD = $\varepsilon$, plug in poly UC rate, to get
Thus have [todo; ignored log m]
\[
m \in \Poly(\frac{1}{\varepsilon^{2}})
\]

Thus approx need $?$

\[
\sqrt{ \mathcal{N}(\varepsilon, \F, \ell_{2}(\ProbDist)) } \leq_{L} \frac{1}{\varepsilon} \enspace?
\]

%So the LB is finite when %$\lim_{\varepsilon \to 0} \dots $


\draftnote{We can use this to show the existence of a polynomial-size cover.
The argument uses Sudakov minorization, see \url{https://www.stat.berkeley.edu/~bartlett/courses/2013spring-stat210b/notes/14notes.pdf}.}
\todo{$\Rade_{m} \in \LandauO_{m}(\Gauss)$, $\Gauss_{m} \in \LandauO(\ln(m)\Rade_{m})$.  If entr function is concave, then largest rectangle and area are similar?}



\end{property}
\fi
\fi

\todo{Dead conjecture: conditions for it holding?}
\if 0 
\begin{conjecture}
Suppose $\F$ is uniformly convergent, and there exists some $\ProbDist$ such that $\exists f \in \F$ with $\Var_{\ProbDist}[f] > 0$.\draftnote{This might require a discrete-valued loss function?}
Then
\[
\sup_{\ProbDist} \Expect_{\bm{x} \distributed \ProbDist^{m}}\left[ \sup_{h \in \HC} \abs{  \ERisk(h; \LossFunction, \bm{x}) - \Risk(h; \LossFunction, \ProbDist) } \right] \in \sup_{\ProbDist} [\mathsmaller{\frac{1}{2}}, 2] \Rade_{m}\bigl( \LossFunction \circ \HC - \Expect_{\ProbDist}[\LossFunction \circ \HC], \ProbDist \bigr) \enspace,
\]
thus \todo{either 0, constant, slow rate.}
\[
\sup_{\ProbDist} \Expect_{\bm{x} \distributed \ProbDist^{m}}\left[ \sup_{h \in \HC} \abs{  \ERisk(h; \LossFunction, \bm{x}) - \Risk(h; \LossFunction, \ProbDist) } \right] \in \LandauTheta \frac{1}{\sqrt{m}} \enspace.
\]
\todo{Prove rate can't be anything else?  Need particular rate for poly SC results.}

\todo{Why this form?  Fast learning does not exist (uniformly).  Is that true for all loss functions?}

\draftnote{False: in regression example, it's $\frac{1}{2^{\LandauOmega(m)}}$?}

\end{conjecture}

\draftnote{This should further imply an equality with \emph{uniform covering numbers}, via the majorizing measures argument (assuming boundedness)?}
\fi


\todo{Note that UC quantified by many dimension quantities for classification, regression, etc.}

It is in general true %\todo{is it?} 
%true for binary classification 
%that \emph{polynomial-rate uniform convergence}
that \emph{uniform convergence} implies \emph{PAC-learnability}; this is well-known for binary classification, but we show the generalized result for completeness.
The converse is true for some learning problems, but not for others, which we shall use as a powerful tool to characterize when PAC-learnability implies fair-PAC-learnability.
\todo{Not sure, now that poly is assumed?  Or does it work, because we had PAC =/=> UC, which implies PAC =/=> poly UC?}
%\begin{lemma}
%\end{lemma}





%TODO: DISCUSS

We first state the fundamental theorem of statistical learning (for classification) \citep[thms.\ 6.2,~29.3]{shalev2014understanding}.\todo{; not .?}


\begin{theorem}[Fundamental Theorem of Statistical Learning (Classification)]
Suppose $\LossFunction$ is the 0-1 loss for $k$-class classification, where $k < \infty$.
%Suppose also $k < \infty$, and the Natarajan dimension $d$ of $\HC$ is also finite.
Then the following are equivalent.
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\HC$ has the uniform convergence property.
\item Any ERM rule is a successful agnostic-PAC learner for $\HC$.
\item $\HC$ is agnostic-PAC learnable.
\item $\HC$ is realizable-PAC learnable.
\item Any ERM rule is a successful realizable-PAC learner for $\HC$.
\item $\HC$ has a finite Natarajan-dimension (= VC dimension for $k=2$ classes).
\end{enumerate}
%\draftnote{Should I generalize to arbitrary learning problems (arbitrary $\LossFunction$)?}
\end{theorem}


It is somewhat subtle to generalize this result to arbitrary learning problems.
In particular, there are PAC-learnable problems for which uniform convergence \emph{does not hold}.\todo{I'm not sure about this: Similarly there are cases where uniform convergence holds but not any ERM rule is capable of agnostic pack learning? Infinite classes?}

\todo{Discuss NFL}
\if 0
In order to obtain a similar result, we require sufficient conditions for a \emph{no-free lunch theorem} for general learning (statistical estimation) problems.
The following suffices, adapted from the classification version given by \citep[thm.~5.1]{shalev2014understanding}.
\begin{theorem}[No Free Lunch Theorem]

Suppose ...

\todo{Check remark 7.2.}
\todo{write me.}




Corollary:

$(\HC, \LossFunction) \in \PAC \implies (\HC, \LossFunction) \in \UC$


\end{theorem}

\draftnote{Actually just need that $\exists \gamma$ s.t. $\VC( \{ x \mapsto \1_[0,\gamma] \LossFunction(h(x), y) \, | \, h \in \HC \} ) < \infty$?  Might need relationship between $\gamma$, $\epsilon$ for polynomial? Anyway, that gives us VC infinite $\implies$ not agnostic PAC?  Thus ag PAC $\implies$ VC finite.  But does this imply UC?  No, it does not.  Need similar for all $\gamma$-cover:, $\VC( \{ x \mapsto \1_[i\gamma,(i+1)\gamma] \LossFunction(h(x), y) \, | \, h \in \HC, i \in \N \} ) < \infty$; looking a bit like PDIM or fat-shattering?  Does this do anything?  How does NFL reduction look?}
\fi

\todo{Discuss Natarajan, graph, pseudo?}


\begin{theorem}[Fundamental Theorem of Fair Statistical Learning]
\label{thm:ftfsl}
\if 0

PAC implies Fair PAC

Non-constructive proof.

May need stronger assumption: something like PAC by ERM implies fair PAC by EMM?

Adapt FTSL (classification, natarajan)?  Regression?




Suppose boundedness (needed for UC to be needed?).
\fi


Suppose $\LossFunction$ such that $\forall \HC: \, (\HC, \LossFunction) \in \PAC^{\Realizable} \implies (\HC, \LossFunction) \in \UC$.
Then, for any hypothesis class sequence $\HC$, the following are equivalent:
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item \label{ftfsl:uc} $\HC$ has the uniform convergence property.\todo{poly?}
\item \label{ftfsl:ag-emm} Any EMM rule is a successful agnostic-fair-PAC learner for $\HC$.
\item \label{ftfsl:ag} $\HC$ is agnostic-fair-PAC learnable.
\item \label{ftfsl:re} $\HC$ is realizable-fair-PAC learnable.
\item \label{ftfsl:re-emm} Any EMM rule is a successful realizable-fair-PAC learner for $\HC$.
%\item $\HC$ has a finite VC-dimension.
\end{enumerate}
%
\todo{What changes if we instead assume $\forall \HC: \, (\HC, \LossFunction) \in \PAC^{\Agnostic} \implies (\HC, \LossFunction) \in \UC$?  I think we just lose 3 and 4?  Or can we show that the conditions are identical? Update 1: I think it's the same.  Update 2: I think we lose everything, since we used NFL for agnostic learning.}
%
\end{theorem}
\begin{proof}
%
First note that \ref{ftfsl:uc} $\implies$ \ref{ftfsl:ag-emm} is a rather straightforward consequence of the definition of uniform convergence and the Lipschitz properties of fair malfare functions.  \draftnote{More detail required.}


\ref{ftfsl:ag-emm} $\implies$ \ref{ftfsl:ag} is almost tautological, and \ref{ftfsl:re-emm} $\implies$ \ref{ftfsl:re} is the same argument. \todo{Need converse of the latter.}

\ref{ftfsl:ag} $\implies$ \ref{ftfsl:re} holds, as realizable learning is a special case of agnostic learning.

The difficult part is to show that \ref{ftfsl:re} $\implies$ \ref{ftfsl:uc}, i.e., if $\HC$ is realizable fair PAC learnable, then $\HC$ has the uniform convergence property.
In general, the question is rather subtle, but here the assumption ``suppose $\LossFunction$ such that $(\HC, \LossFunction) \in \PAC^{\Realizable} \implies (\HC, \LossFunction) \in \UC$'' does all of the work.
In particular, by \cref{obs:pac2fpac} we have that $(\HC, \LossFunction)$ in $\FPAC^{\Agnostic}$ implies $(\HC, \LossFunction)$ in $\PAC^{\Agnostic}$, then applying the assumption yields $(\HC, \LossFunction) \in \UC$.
%
\todo{New:
If $\abs{\X}$ is finite, then ?
\ref{ftfsl:re}: $\HC$ is realizable fair PAC learnable implies $\HC$ is realizable PAC learnable.
}
%
\end{proof}
The reductions and equivalences that compose this result are graphically depicted in \cref{fig:ftfsl}.

\begin{observation}[The Gap Between Uniform Convergence and (fair) PAC-Learnability]
Note that the assumption ``suppose $\LossFunction$ such that $(\HC, \LossFunction) \in \PAC^{\Realizable} \implies (\HC, \LossFunction) \in \UC$'' does not in general hold.

In many cases of interest, it is known to hold, e.g., finite-class classification under 0-1 loss, (bounded?) regression under square and absolute loss.
It is known to not hold in some more obscure cases.

Verifying this condition is a rather subtle task, and until more general techniques are developed, must be repeated for each learning problem (loss function).
\todo{Can we better characterize this dichotomy?  What about density estimation and recommender systems?}
%
\todo{Furthermore, the gap for PAC-learnability implies a similar gap for fair-PAC-learnability. \draftnote{Reduction goes here.}}
\end{observation}

The following conjecture better characterizes this gap in one direction.
\begin{conjecture}
\label{conj:ftsl-gap-nfl}
%The following suffices, adapted from the classification version given by \citep[thm.~5.1]{shalev2014understanding}.
If the learning problem defined by $\LossFunction$ has a \emph{no free lunch} argument, analogous to \citep[thm.~5.1]{shalev2014understanding}, then the assumption ``suppose $\LossFunction$ such that $(\HC, \LossFunction) \in \PAC^{\Realizable} \implies (\HC, \LossFunction) \in \UC$'' holds.
An additional condition may be required to ensure that $(\HC, \LossFunction) \not\in \UC \implies (\HC, \LossFunction) \not\in \PAC^{\Agnostic}$, as the standard FTSL argument is specific to \emph{shattering} infinite sets (and thus the VC dimension).

\draftnote{Essentially, we need that for non uniformly-convergent classes, there exists a distribution $\ProbDist$ over $2m$ points, such that conditioning on $m$ samples (ERM training) doesn't tell us much about the remaining $m$ samples.
I think a covering number argument gets us here, using the $\gamma$-fat-shattering dimension.}
\end{conjecture}
%
\todo{
An alternate condition, which should also be sufficient for bounded $\LossFunction$, would be to define the \emph{discretization loss class}
\[
\F_{\varepsilon} \doteq \{ x \mapsto \1_[0,\varepsilon] \LossFunction(h(x), y) \, | \, h \in \HC \} \enspace,
\]
and then require that $\forall \varepsilon > 0$, $\VC( \F_{\varepsilon} ) < \infty$ (approaching the limit sufficiently slowly).
This class is closely related to the \emph{pseudo-dimension} or the $\gamma$-\emph{fat-shattering dimension}.
The 0-1 loss used by $\F_{\varepsilon}$ can be used to upper and lower bound the $\LossFunction$ loss of $\F$, rather coarsely, but finely enough to apply the standard binary-classification NFL result to complete the fundamental theorem of statistical learning.
Intuitively, this seems more stringent (and far less elegant) than \cref{conj:ftsl-gap-nfl}, but it remains unclear whether either condition is \emph{necessary}.
}
\todo{Proof with this?
Overview: show that if $\PacAlgo$ realizable PAC-learns $\F$, then exists $\PacAlgo'$ to realizable PAC-learn $\F_{\gamma}$, thus $\F_{\gamma}$ is UC.
Also, if $\F$ is UC, then $\F_{\gamma}$ is UC.
Start by assuming $\F \not \in \UC$.
Apply double-contrapositive: $\F_{\gamma} \not \in \UC \implies \F \not \in \UC$, and also $\F_{\gamma} \not \in \UC \implies \F_{\gamma} \not \in \PAC^{\Realizable} \implies \F \not \in \PAC^{\Realizable}$.
Doesn't work: need $\F_{\gamma} \in \UC \implies \F \in \UC$.
Alt strategy:
Assume $\F \in \PAC^{\Realizable}$.  Then $\F_{\gamma} \in \UC$ (again need $\F_{\gamma} \in \UC \implies \F \in \UC$).
The fix:
In both cases, consider multiple values of $\gamma$.  Looking more like the PDIM then.
}
\todo{So it's not quite right; I think we need pdim?}
%  Take $\gamma \doteq \varepsilon/\frange$ and perform PAC-learning on $\F_{\gamma}$}


\todo{Silly example: can we construct $\HC$ such that ``part of'' $\HC$ is not uniformly convergent, but always has higher loss than all else?  Yes, but not uniformly over any distribution for sensical symmetric loss?  $\X = \Y = [0, 1]$, $\LossFunction(y, \hat{y}) = \hat{y}$.  Now take $\HC \doteq \{ x \mapsto \gamma x | \gamma \in (0, 1) \} \union ([0, 1] \to [\frac{1}{2}, 1])$. %\hat{y} - y + \1_{[1/2,1]}(\hat{y})$, }
Ridiculous, but seems to be a problem?}


\todo{Instances where it doesn't hold: factored loss $\LossFunction(y, h(x)) \doteq \LossFunction_{1}(y_{1}, h_{1}(x_{1})) + \LossFunction_{2}(y_{2}, h_{2}(x_{2}))$.
Take $\HC = \HC_{1} \times \{x \mapsto \1_{I}(x) \, | \, I \subseteq \X \}$, $\Loss_{2}(y, h_{2}(x) \doteoq h_{2}(x)$.
For $\ProbDist$ uniform over $\X \doteq [0, 1]$, ``most'' ERM are ``bad'' ERM; good ERM always takes $h_{2}(x) \detq \1_{\emptyset}(x)$.
Not UC, not learnable by any ERM, but learnable by an ERM.
}


\todo{GOAL, BUT VERY HARD: Can we show that $\PAC = \FPAC$, even when the assumption does not hold?  In other words, if PAC (but not by ERM, i.e., no UC), then fair PAC (pretty tricky)?  Furthermore, if not PAC, then not FPAC (trivially true)?}


\begin{SCfigure}[0.72]

\colorlet{pcol}{red}
\colorlet{fpcol}{blue}
\colorlet{uccol}{brown}

\null\hspace{-0.25cm}\begin{tikzpicture}[
    xscale=2.0,yscale=1.5,
    class/.style={rectangle,draw,thick,rounded corners=0.5ex},
    grouping/.style={rectangle,draw,very thick,rounded corners=1.5ex,inner sep=1ex},
    imp/.style={line width=0.4mm,-implies,double equal sign distance},
    equiv/.style={line width=0.4mm,implies-implies,double equal sign distance},
    ucclass/.style={class,fill=uccol!20!white},
    pclass/.style={class,fill=pcol!15!white},
    fpclass/.style={class,fill=fpcol!15!white},
  ]


%UC:
%\node (ucspace) at (3,3) {};
\node[ucclass] (uc) at
  %(1, 2)
  (0, 2)
  { $\UC(\LossFunction)$ \vspace{1cm} \null};
\node[ucclass] (dim) at
  %(4, 2)
  (2.5, 2)
  { \begin{tabular}{c} Finite \\ Natarajan / VC \\ dimension \\ \end{tabular} };

%TODO: opacity, sth like fill=uccol!5!white, need to draw box below everything.
\node[grouping,fit={(uc) (dim) (3,2.9)},draw=black] (ucgroup) {};
\node[above = -0.6cm of ucgroup] (uctitle) {\bf \color{uccol!50!black} Uniform Convergence};


%Agnostic:
\node[pclass] (pac) at (0, 0) { $\PAC(\LossFunction)$ };
\node[fpclass] (fpac) at (2, 0) { $\FPAC(\LossFunction)$ };

\node[pclass] (pac-erm) at (0, 1) { $\PAC(\LossFunction)$ ERM };
\node[fpclass] (fpac-emm) at (2, 1) { $\FPAC(\LossFunction)$ EMM };

\node[grouping,fit=(pac) (fpac) (pac-erm) (fpac-emm),draw=black] {\bf Agnostic Learning};


%Realizable:
\node[pclass] (rpac) at (0, -2) { $\PAC^{\Realizable}(\LossFunction)$ };
\node[fpclass] (rfpac) at (2, -2) { $\FPAC^{\Realizable}(\LossFunction)$ };

\node[pclass] (rpac-erm) at (0, -1) { $\PAC^{\Realizable}(\LossFunction)$ ERM };
\node[fpclass] (rfpac-emm) at (2, -1) { $\FPAC^{\Realizable}(\LossFunction)$ EMM };

\node[grouping,fit=(rpac) (rfpac) (rpac-erm) (rfpac-emm),draw=black] {\bf Realizable Learning};


%More Labels:
\node at (0, -2.5) {\bf \color{pcol!50!black} PAC Learning};

\node at (2, -2.5) {\bf \color{fpcol!50!black} Fair PAC Learning};


%TODO nodes over implications?

%Implication edges (Organized by source):

%UC:

\draw[imp] (uc) -- (fpac-emm);
\draw[imp] (uc) -- (pac-erm);

\draw[equiv,dashed] (dim) -- node[above] { \begin{tabular}{c} 0-1 loss \\ $k < \infty$ classes \\ \end{tabular} } (uc);

%FTSL
%\draw[imp] (uc) -- (rfpac-emm);
%\draw[imp] (uc) -- (rpac-erm);


%Agnostic:

\draw[imp] (fpac) -- (pac);
\draw[imp] (fpac-emm) -- (pac-erm);

\draw[imp] (fpac-emm) -- (fpac);
\draw[imp] (pac-erm) -- (pac);



\draw[imp] (fpac-emm) .. controls (3, 0) .. (rfpac-emm);
\draw[imp] (pac-erm) .. controls (-1, 0) .. (rpac-erm);

\draw[imp] (fpac) .. controls (3, -1) .. (rfpac);
\draw[imp] (pac) .. controls (-1, -1) .. (rpac);

%Realizable:

%\draw[imp] (rfpac) -- (rpac);
%\draw[imp] (rfpac-emm) -- (rpac-erm);
\draw[equiv] (rfpac) -- (rpac);
\draw[equiv] (rfpac-emm) -- (rpac-erm);

%TODO: poly time reverse arrows.



\draw[imp] (rfpac-emm) -- (rfpac);
\draw[imp] (rpac-erm) -- (rpac);



\draw[imp,dashed] (rpac) .. controls  (-2, -2) and (-2, 2) .. node[left of=-0.5cm,xshift=0.6cm,yshift=0.2cm,rotate=86] { Assumption on $\LossFunction$ }
  %{ \begin{tabular}{c} $\LossFunction$ Satisfies \\ ??? \\ \end{tabular} }
  (uc);


\end{tikzpicture}


\caption{Implications between membership in various PAC and fair-PAC classes.  In particular, for arbitrary but fixed $\LossFunction$, implication denotes \emph{implication of membership} of some $\HC$ (i.e., containment). See \cref{thm:ftfsl,thm:ftfsl}, as well as \cref{thm:realizable-pac2fpac}.
Dashed implication arrows hold conditionally on $\LossFunction$.
Note that when the assumption on $\LossFunction$ (see \cref{thm:ftfsl}) holds, the hierarchy collapses, and in general, under realizability, some classes are known to coincide.}
%Fundamental Theorem of Fair Statistical Learning
%\caption{Fundamental Theorem of Fair Statistical Learning}
\label{fig:ftfsl}

\todo{Grouping to classic document.}
\todo{$(\HC, \LossFunction) \in$ notation}
\end{SCfigure}

\todo{Can graph dim relax infinite class count issue?}

\todo{Collapse hierarchy of $\F$? Only in realizable case?}


\todo{Is k-NN PAC learnable?}

\subsection{Characterizing Computational Learnability}%TODO SECTION:

\todo{Example: linear classifier / regressor; both coverable efficiently for fixed $d$, but expo in $d$.}


\todo{Restore fig.}
\if 0
\begin{SCfigure}[0.5]

\colorlet{uccol}{brown}
\colorlet{cocol}{green!50!black}

\colorlet{pcol}{red}
\colorlet{fpcol}{blue}

\null\hspace{-0.25cm}\begin{tikzpicture}[
    xscale=2.0,yscale=1.5,
    class/.style={rectangle,draw,thick,rounded corners=0.5ex},
    grouping/.style={rectangle,draw,very thick,rounded corners=1.5ex,inner sep=1ex},
    imp/.style={line width=0.4mm,-implies,double equal sign distance},
    equiv/.style={line width=0.4mm,implies-implies,double equal sign distance},
    ucclass/.style={class,fill=uccol!20!white},
    coclass/.style={class,fill=cocol!20!white},
    pclass/.style={class,fill=pcol!15!white},
    fpclass/.style={class,fill=fpcol!15!white},
  ]


%UC:
%\node (ucspace) at (3,3) {};
\node[ucclass] (uc) at
  %(1, 2)
  (0, 2)
  { $\UC(\LossFunction)$ \vspace{1cm} \null};
\node[ucclass] (dim) at
  %(4, 2)
  (2.5, 2)
  { \begin{tabular}{c} Finite \\ Natarajan / VC \\ dimension \\ \end{tabular} };

\node[ucclass] (efficient-covering) at
  %(4, 2)
  (5, 2)
  { \begin{tabular}{c} Efficient \\ Covering \\ \end{tabular} };

%TODO: opacity, sth like fill=uccol!5!white, need to draw box below everything.
\node[grouping,fit={(uc) (dim) (efficient-covering) (3,2.9)},draw=black] (ucgroup) {};
\node[above = -0.6cm of ucgroup] (uctitle) {\bf \color{uccol!50!black} Uniform Convergence};


%Convexity

\node[coclass] (co) at
  %(1, 2)
  (6, 2)
  { Convex Optimization }; % $\UC(\LossFunction)$ \vspace{1cm} \null};
\node[coclass] (dim) at
  %(4, 2)
  (7, 2)
  { \begin{tabular}{c} Convex \\ Lipschitz \\ Bounded \\ Evaluable \\ Self-Concordancy? \\ \end{tabular} };


%Agnostic:
\node[pclass] (pac) at (0, 0) { $\PAC_{\Poly}(\LossFunction)$ };
\node[fpclass] (fpac) at (2, 0) { $\FPAC_{\Poly}(\LossFunction)$ };

\node[pclass] (pac-erm) at (0, 1) { $\PAC_{\Poly}(\LossFunction)$ ERM };
\node[fpclass] (fpac-emm) at (2, 1) { $\FPAC_{\Poly}(\LossFunction)$ EMM };

\node[grouping,fit=(pac) (fpac) (pac-erm) (fpac-emm),draw=black] {\bf Agnostic Learning};


%Realizable:
\node[pclass] (rpac) at (0, -2) { $\PAC_{\Poly}^{\Realizable}(\LossFunction)$ };
\node[fpclass] (rfpac) at (2, -2) { $\FPAC_{\Poly}^{\Realizable}(\LossFunction)$ };

\node[pclass] (rpac-erm) at (0, -1) { $\PAC_{\Poly}^{\Realizable}(\LossFunction)$ ERM };
\node[fpclass] (rfpac-emm) at (2, -1) { $\FPAC_{\Poly}^{\Realizable}(\LossFunction)$ EMM };

\node[grouping,fit=(rpac) (rfpac) (rpac-erm) (rfpac-emm),draw=black] {\bf Realizable Learning};


%More Labels:
\node at (0, -2.5) {\bf \color{pcol!50!black} PAC Learning};

\node at (2, -2.5) {\bf \color{fpcol!50!black} Fair PAC Learning};


%TODO nodes over implications?

%Implication edges (Organized by source):

%UC:

\draw[imp] (uc) -- (fpac-emm);
\draw[imp] (uc) -- (pac-erm);

\draw[equiv,dashed] (dim) -- node[above] { \begin{tabular}{c} 0-1 loss \\ $k < \infty$ classes \\ \end{tabular} } (uc);

%FTSL
%\draw[imp] (uc) -- (rfpac-emm);
%\draw[imp] (uc) -- (rpac-erm);


%Agnostic:

\draw[imp] (fpac) -- (pac);
\draw[imp] (fpac-emm) -- (pac-erm);

\draw[imp] (fpac-emm) -- (fpac);
\draw[imp] (pac-erm) -- (pac);



\draw[imp] (fpac-emm) .. controls (3, 0) .. (rfpac-emm);
\draw[imp] (pac-erm) .. controls (-1, 0) .. (rpac-erm);

\draw[imp] (fpac) .. controls (3, -1) .. (rfpac);
\draw[imp] (pac) .. controls (-1, -1) .. (rpac);

%Realizable:

%\draw[imp] (rfpac) -- (rpac);
%\draw[imp] (rfpac-emm) -- (rpac-erm);
\draw[equiv] (rfpac) -- (rpac);
\draw[equiv] (rfpac-emm) -- (rpac-erm);

%TODO: poly time reverse arrows.



\draw[imp] (rfpac-emm) -- (rfpac);
\draw[imp] (rpac-erm) -- (rpac);



\draw[imp,dashed] (rpac) .. controls  (-2, -2) and (-2, 2) .. node[left of=-0.5cm,xshift=0.6cm,yshift=0.2cm,rotate=86] { Assumption on $\LossFunction$ }
  %{ \begin{tabular}{c} $\LossFunction$ Satisfies \\ ??? \\ \end{tabular} }
  (uc);


\end{tikzpicture}


\caption{
%Implications between membership in various PAC and fair-PAC classes.  In particular, for arbitrary but fixed $\LossFunction$, implication denotes \emph{implication of membership} of some $\HC$ (i.e., containment). See \cref{thm:ftfsl,thm:ftfsl}, as well as \cref{thm:realizable-pac2fpac}.
%Dashed implication arrows hold conditionally on $\LossFunction$.
%Note that when the assumption on $\LossFunction$ (see \cref{thm:ftfsl}) holds, the hierarchy collapses, and in general, under realizability, some classes are known to coincide.
}
%Fundamental Theorem of Fair Statistical Learning
%\caption{Fundamental Theorem of Fair Statistical Learning}
\label{fig:fclt}

\todo{Grouping to classic document.}
\todo{$(\HC, \LossFunction) \in$ notation}
\end{SCfigure}
\fi




\paragraph{Realizability}

We now show that in the \emph{realizable case}, \emph{PAC-learnability} implies \emph{fair PAC-learnability}.
In particular, we employ a simple and practical \emph{constructive} polynomial-time reduction.
More efficient reductions are possible for particular values of $p$, $\NGroups$\todo{Weights}.\todo{More efficient if can change loss function; e.g., loss is avg or worst-case over a per-group sample.  But this may require a different assumption.}
Our reduction simply takes a sufficiently (polynomially large) number of samples from the \emph{uniform mixture distribution} over all $\NGroups$ groups, and PAC-learns on this distribution.
%Form PAC learning with guarantee $\epsilon$ over $\NGroups$ and $\delta$. The result has L infinity norm bound $\epsilon$ which implies P welfare bound $\epsilon$.

\todo{Call it a property?}
\begin{theorem}[Realizable Reductions]
\label{thm:realizable-pac2fpac}
Suppose $(\HC, \LossFunction)$ is (efficiently) \emph{realizable-PAC-learnable}.
Then $(\HC, \LossFunction)$ is (efficiently) \emph{realizable-PAC-learnable}.
%Furthermore, 

In particular, there exists $\PACAlgo$ with (sample / time)-complexity $C(\varepsilon, \delta)$ to PAC-learn $(\HC, \LossFunction)$, and we may take $\PACAlgo'(p, \wv, \ProbDist_{1:\NGroups}, \varepsilon, \delta, \DSeq) \doteq \PACAlgo(\mix(\ProbDist_{1:\NGroups}),\nicefrac{\varepsilon}{\NGroups}, \delta, \DSeq)$.
Then $\PACAlgo'$ fair-PAC-learns $(\HC, \LossFunction)$, with (sample / time)-complexity $C_{\PACAlgo'}(\varepsilon, \delta, \DSeq, \NGroups) = C_{\PACAlgo}(\nicefrac{\varepsilon}{\NGroups}, \delta, \DSeq)$.
\todo{Minor issue on whether sample complexity can depend on $\NGroups$.}
\end{theorem}
\begin{proof}
We first show the sample complexity result.
%Suppose $\hat{h}$ returned by $\PACAlgo$'.
Suppose $\hat{h} \gets \PACAlgo'(p, \wv, \ProbDist_{1:\NGroups}, \varepsilon, \delta, \DSeq)$.
Then, with probability at least $1 - \delta$ (by the guarantee of $\PACAlgo$), we have
\begin{align*}
\Malfare_{p}( i \mapsto \Risk(h; \LossFunction, \ProbDist_{i})), \wv)
 &\leq \Malfare_{\infty} \bigl( i \mapsto \Risk(h; \LossFunction, \ProbDist_{i}), i \mapsto \mathsmaller{\frac{1}{\NGroups}}\bigr) & \\
 &= \Malfare_{\infty} \bigl( i \mapsto \Risk(h; \LossFunction, \ProbDist_{i}), i \mapsto \mathsmaller{\frac{1}{\NGroups}}\bigr) & \\
 &\leq \NGroups \Malfare_{1} \bigl( i \mapsto \Risk(h; \LossFunction, \ProbDist_{i}), i \mapsto \mathsmaller{\frac{1}{\NGroups}}\bigr) & \\
 &= \NGroups \Risk \bigl(h; \LossFunction, \mix(\ProbDist_{1:\NGroups}) \bigr) & \\
 &\leq \NGroups \mathsmaller{\frac{\varepsilon}{\NGroups}} = \varepsilon \enspace. & \\
\end{align*}
We thus may conclude that $(\HC, \LossFunction)$ is (efficiently) \emph{realizable-PAC-learnable} by $\PACAlgo'$, with \emph{sample complexity} $C_{\PACAlgo}(\nicefrac{\varepsilon}{\NGroups}, \delta, \DSeq)$.

Similarly, if $\PACAlgo$ has polynomial runtime, then so too does $\PACAlgo'$, thus we may also conclude efficiency.\todo{Justifications}
%
\end{proof}

\todo{Explain why it's philosophically an uninteresting fairness concept.  Conflict.}

\todo{Observe?}
\if 0
\begin{observation}
per-group realizability is much stronger, and (realizable) PAC doesn't imply it.
\end{observation}
\fi

\todo{Note that the reduction can't really be improved for $p=\infty$; since in realizable, SC $\propto 1/\varepsilon' = \NGroups/\varepsilon$, and obviously need factor $\NGroups$, since if all but one group is trivially satisfiable, only last group matters?}

%TODO: Idea loosely based on uml 13.7 EX 1 (not really): if 0 error on all groups, then w.h.p., roughly $\nicefrac{\delta}{\NGroups}$, per-group.


\todo{If 0-neighborhoods of $\LossFunction'$ contain 0-neighborhoods of $\LossFunction$ (w.r.t., $\hat{y}$), then PAC on $\LossFunction$ implies PAC on $\LossFunction'$ in realizable case. Agnostic form?}

\todo{GRID REDUCTION: fair-PAC-learnable, but not by ERM; is it unstable?}



\draftnote{I'm omitting discussion of computational learning theory for agnostic PAC learning for now.}









\if 0

\todo{Convex optimization, efficiently enumerable uniform convergence, and stable optimization with grid search?}


\subsection{Convex Optimization}

Convex, Lispchitz, bounded, finite dimension, constant time evaluable gradient approx (implied by ctime value approx)

Is that enough?

pmean preserves all of these?  $\infty$ breaks smoothness though?


Self-concordancy: \url{https://en.wikipedia.org/wiki/Self-concordant_function}.  See \url{https://www.wolframalpha.com/input/?i=d%5E3%2Fdx%5E3+%28x%5Ep+%2B+1%29%5E%281%2Fp%29}  Use this: \url{https://www.wolframalpha.com/input/?i=d%2Fdx+%28x%5Ep+%2B+1%29%5E%281%2Fp%29}?


What we need: cover is polynomial size in dimension; optimizer needs to cut out a constant amount per step?



TODO: ALSO SUBMODULAR?


Composition of convex $\Malfare$ w/ convex $\theta$?  Tricky because multivariate.



\subsection{Convex Lipschitz Bounded}

See

ELEG/CISC 867: Advanced Machine Learning
Spring 2019
Lecture 9: Convex Learning Problems
Lecturer: Xiugang Wu


CLB is good.
$\beta$-smooth, for some reason means gradient is $\beta$-Lipschitz.

Strongly convex: stronger than strict \url{https://en.wikipedia.org/wiki/Convex_function#Strongly_convex_functions}



\subsection{Uniform Convergence and Efficient Covering}
\label{sec:time:uc}
As we have seen in \cref{sec:ftfsl}, uniform convergence implies, and is often equivalent to, (fair) PAC-learnability.
However, these results all consider only \emph{statistical learning}, and to analyze \emph{computational learning} questions, we introduce a strengthening of uniform convergence that considers \emph{computation}.

In particular, in the case where PAC-learnability and UC are equivalent, we show that if a \emph{cover} of $\F$ may be efficiently enumerated, then $(\HC, \LossFunction) \in \FPAC_{\Poly}$.


\draftnote{Result 2.  Uniform convergence implies fair pack or nobility. Plus efficient innumerabilis I implies efficient fair. Q:  Does this mean pack implies fair pack?
  ALWAYS TRUE THAT UC => PAC (citation), but EX WHERE PAC =/=> UC.  
  However, when $PAC = UC$, then PAC =/=> Fair-PAC.
}

%We also show that PAC-learnability implies a generic poly-time routine when a \emph{cover} of $\F$ may be efficiently enumerated.


\begin{lemma}[Uniform Convergence and Efficient Enumerability]
\label{cor:uc-eff}

Suppose any $\bm{x} \in \X^{m}$, and denote the projection of $\F$ onto $\HC$ as $\F(\bm{x}) \in \R^{m}$.



\draftnote{OLD:
\color{green!50!black}

Suppose $\HC$ has finite VC-dimension $d$, and the \emph{projection} of $\HC$ onto $\bm{x} \in \X^{m}$ can be enumerated in $\Poly(m)$ time (wherein $d$ is a constant).
Then $\HC$ is fair-PAC-learnable.

Furthermore, suppose generic $\HC \subseteq \X \to \Y$, $\loss \in \Y \times \Y \to [0, 1]$, and assume that\todo{Scaling?}
\begin{enumerate}[wide, labelwidth=0pt, labelindent=0pt]\setlength{\itemsep}{3pt}\setlength{\parskip}{0pt}
\item $\Y$ is a set of diameter $D_{\Y}$, and $\loss$ is $\lambda_{\loss}$-Lipschitz continuous;
\item the $\ell_{2}$ covering number%
\footnote{The reader is invited to consult \citep{anthony2009neural} for an encyclopedic overview of various covering numbers and their applications to statistical learning theory.}
$\mathcal{N}(\HC, \bm{x}, \gamma) \in \Poly(m, \nicefrac{1}{\gamma})$;
\item a \emph{$\gamma$-precision cover} $\mathcal{C}(\HC, \bm{x}, \gamma)$ of size $\LandauO(\mathcal{N}(\HC, \bm{x}, \gamma))$ may be enumerated in $\Poly(m, \nicefrac{1}{\gamma})$ time.
\end{enumerate}
Then $\HC$ is efficiently fair-PAC-learnable.
Items (1) and (2) are sufficient to show that $\HC$ is fair-PAC learnable; (3) is required only to show \emph{efficiency}.

}

Suppose there exists a routine $\UCAlgo$ that \emph{enumerates} a $\gamma$-\emph{cover} of [...] of size $\LandauTheta( \mathcal{N}(\HC, \bm{x}, \gamma) )$, where each \emph{enumeration step} requires $\Poly(\dots)$ time.

If $(\HC, \LossFunction) \in \UC$, then enumerating \emph{all of} $\UCAlgo$ requires $\Poly(\dots)$ time, and furthermore, we may employ $\UCAlgo$ as a subroutine in constructing a $\PACAlgo$ to PAC-learn $(\HC, \LossFunction)$ in polynomial time, i.e., $(\HC, \LossFunction) \in \FPAC_{\Poly}$

\end{lemma}
\begin{proof}

We first show that $\UCAlgo$ may be run to completion in polynomial time.
\todo{majorizing measures: Gaussian avg <= (...) * Rade avg, GA bounds cover size as poly, poly * poly is poly.}

We now construct a $\PAC_{\Poly}$ algorithm given $\UCAlgo$.
\todo{Select $\gamma$, enumerate cover, ERM over cover.}

\end{proof}

\begin{corollary}[Uniform Convergence, PAC-Learning, and Poly-Time Learnability]
\label{cor:uc-ftsl}
%If $\UC(\HC, \LossFunction) = \PAC(\HC, \LossFunction)$, then $\PAC(\HC, \LossFunction) \implies \FPAC(\HC, \LossFunction)$.

If $\UC(\LossFunction) = \PAC(\LossFunction)$, then $(\HC, \LossFunction) \in \PAC \implies (\HC, \LossFunction) \in \FPAC$. [Thus $\PAC(\LossFunction) = \FPAC(\LossFunction)$]

Furthermore, $(\HC, \LossFunction) \in \UC_{\Poly} \implies (\HC, \LossFunction) \in \FPAC_{\Poly}$.

\todo{and polytime}
\todo{agnostic}

TODO: NOTATION MAKES LITTLE SENSE; SETS NOT FUNCTIONS?
Can parameterize by only $\LossFunction$ to make more sense?  Sth like

\end{corollary}

While \cref{cor:uc-ftsl} may seem a bit tautological, for many notable machine learning tasks (e.g., finite-class classification under $0$-$1$ loss \citep{shalev2014understanding}, regression \citep{?}, etc), it holds that $\UC(\LossFunction) = \PAC(\LossFunction)$.

\begin{conjecture}[Efficient Learning Covering Duality]
\label{conj:poly-uc-poly-pac}
$(\HC, \LossFunction) \in \PAC_{\Poly} \implies (\HC, \LossFunction) \in \UC_{\Poly}$
\end{conjecture}
\begin{consequence}
\label{cons:poly-uc-poly-pac}
Suppose \cref{conj:poly-uc-poly-pac} and $\LossFunction$ such that $\UC(\LossFunction) = \PAC(\LossFunction)$.
Then $(\HC, \LossFunction) \in \PAC_{\Poly} \implies (\HC, \LossFunction) \in \FPAC_{\Poly}$. [Then $\PAC_{\Poly}(\LossFunction) = \FPAC_{\Poly}(\LossFunction)$.]
\begin{consequence}
\begin{proof}
This result follows directly from \cref{conj:poly-uc-poly-pac} and \cref{cor:uc-ftsl}.
\begin{proof}



\begin{observation}

\draftnote{Move me?}

Although it holds $\forall (\HC, \LossFunction)$ that $\UC(\HC, \LossFunction) \implies \PAC(\HC, \LossFunction)$, in general the converse \emph{is not true}.

TODO: NOTE: TRUE FOR 0-1 binary CLASSIFICATION; REGRESSION (sq or abs loss); XXX?

See fundamental theorem of learning theory (thm.~6.2) of \citep{shalev2014understanding}.
TODO: CALL IT ``of statistical learning.''


See also multi-class version, thm. 29.3.  Note: Natarajan only, contrast with graph dim.  Seem to need finite classes, $k < \infty$? Conclusion: PAC = UC.


Nonlearnable: remark~6.3
PROBLEM: their construction is slightly different; I think it's OK if loss is asymmetric. Make note of asym loss?


TODO: Boundedness not sufficient; stability is? Is this what we show?  Or a proof technique we use?


TODO: thm: non-UC but still realizable PAC for regression-type problems: Take $\HC$, union with a non-convergent class that gets everything at least slightly wrong: e.g., if we're doing regression with codomain $[0, 1]$, the non-convergent part of the HC has codomain $\R \setminus [2, 3]$.


\end{observation}




TODO: 6.3 MAKES NO SENSE; DON'T HAVE UC FOR UNBOUNDED LOSS.

NONUNIFORM CONVERGENCE?



uml 13.7 exercise 2:

this mean est has no UC, but is learnable.
fair PAC => PAC =/> UC; use to show fair PAC =/> UC


\begin{observation}
Exist $\HC$ such that enumerating projection is NP-hard.

Reduction: construct $\HC$ s.t. $\hat{h}$ corresponds to soln of an NP-hard decision problem?

Don't see a way to do it without an $\NGroups$ parameter.
\end{observation}


\begin{observation}[Same subject: now parameterizing family.]

MUST EXIST: UC = PAC, and poly enum UC implies (PAC = poly PAC), thus exist UC HC that don't admit poly enum.


EXAMPLES: Note: these assume $\DSeq$ is a parameter!  I call this a ``meta-family'' $\F_{\dots}$.
  Is poly-PAC =/= PAC for fixed HC?  Seems to suggest / imply yes in 8.2.2:
  
  ``On the other hand, it is worthwhile noticing that, if we fix one specific hypoth-
esis class, say, axis aligned rectangles in some fixed dimension, $n$, then there exist
efficient learning algorithms for this class. In other words, there are successful
agnostic PAC learners that run in time polynomial in $\nicefrac{1}{\varepsilon}$ and $\nicefrac{1}{\delta}$ (but their dependence on the dimension n is not polynomial).''

  Boolean conjunctions: \S 8.2.3 of UML.
  Halfspaces (well known).
  Hyperrectangles.
  
  \S 8.4: mentions small Boolean functions.
  
  Neural networks \url{https://papers.nips.cc/paper/125-training-a-3-node-neural-network-is-np-complete.pdf}
  
  \draftnote{Learning real-valued decision trees, depth bounded by sample size, continuous input, may give meaningful example?}
  
\end{observation}

\paragraph{NEW STABILITY}

\todo{Cut me?}

Stability implies \cref{cor:uc-ftsl} condition $\UC(\LossFunction) = \PAC(\LossFunction)$???  does it make sense?

Theoretical consequence, but uses inefficient enumeration ctrn; must enumerate $\HC$ (unknown how).

Alternative ctrn in terms of $\PACAlgo$ (also inefficient in $\NGroups$ though).


\paragraph{The Non-Equivalence Conjecture}

\begin{conjecture}
There exist $(\HC, \LossFunction)$ such that evaluating
\[
\argmin_{\hat{h} \in \HC_{\DSeq}} \ERisk(\hat{h}; \LossFunction, \bm{x})
\]
is NP-hard. \draftnote{Hardness is in $\nicefrac{1}{\varepsilon}, \DSeq$.

\todo{Need something like \whp{} over $\bm{x}$?}

\end{conjecture}
\begin{consequence}
There exist learning problems characterized by $\LossFunction$ such that PAC-learnability does not imply fair-PAC learnability.
Thus we have
\[
\FPAC_{\Poly}(\LossFunction) \subset \PAC_{\Poly}(\LossFunction) \enspace,
\]
i.e., the \emph{fair-PAC-learnable classes} are a \emph{strict subset} of the \emph{PAC-learnable classes}.
\end{consequence}
\begin{proof}
Use fundamental theorem of statistical learning + the conjecture?
\end{proof}
\begin{observation}
This contrasts ???, which shows equivalence under \emph{realizability}.
\end{observation}






\todo{Good stuff below.}

\if 0

\section{Online cost model}

TODO: GENERIC METHOD



\section{Welfare and Lipschitz Constants: Take XVII}

%https://www.wolframalpha.com/input/?i=Simplify+%28w+*+x%5E%28-1+%2B+p%29+*+%28%281-w%29R+%2B+w+x%5Ep%29%5E%28-1+%2B+1%2Fp%29%29%2C+Assuming+x+%3E+0+and+w+%3E+0+and+R+%3E+0

Take $R \doteq \Welfare_{p}^{p}(\lv_{2:\NGroups}, \wv_{2:\NGroups})$ (improper).
\[
\frac{\partial}{\partial \lv_{1}} \Welfare_{p}(\lv; \wv) = \wv_{1} \lv_{1}^{p - 1}(\wv_{1} \lv_{1}^{p} + R(1 - \wv_{1}))^{-1 + 1/p}
\]

\[
= \wv_{1} \lv_{1}^{-(1 - p)}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})R)^{-(1 - 1/p)}
\]

\[
= \left(\wv_{1}^{-1} \lv_{1}^{1 - p}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})R)^{1 - 1/p}\right)^{-1}
\]

Consider extreme values of $R = 0, \frange^{p} < \infty$ By Anti? monotonicity, for $p < 0$, we have

\[
\in \left[ \left(\wv_{1}^{-1} \lv_{1}^{1 - p}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})\infty)^{1 - 1/p}\right)^{-1}, \left(\wv_{1}^{-1} \lv_{1}^{1 - p}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})0)^{1 - 1/p}\right)^{-1} \right]
\]
\[
= \left[ 0, \left(\wv_{1}^{-1} \lv_{1}^{1 - p}(\wv_{1} \lv_{1}^{p})^{1 - 1/p}\right)^{-1} \right]
\]

\[
= \left[ 0, \wv_{1}^{\frac{1}{p}} \right] \enspace.
\]

Consequently, for $p < 0$, we have that $\Welfare_{p}$ is $\Mean_{-\infty}^{\frac{1}{p}}(\wv)$-Lipschitz w.r.t. $\norm{\cdot}_\infty$.


Hessian: %\url{https://www.wolframalpha.com/input/?i=Hessian+of+%28x%5Ep%2F2+%2B+y%5Ep%2F2%29%5E%281%2Fp%29}
More Hessian: %\url{https://www.wolframalpha.com/input/?i=Eigenvalues+of+HessianMatrix%5B%28x%5Ep+%2B+y%5Ep%29%5E%281%2Fp%29%5D}


\subsection{The Bad Case}

For $p \in (0, 1)$, we have
\[
\in \left[ \left(\wv_{1}^{-1} \lv_{1}^{1 - p}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})0 )^{1 - 1/p}\right)^{-1}, \left(\wv_{1}^{-1} \lv_{1}^{1 - p}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})\frange^{p} )^{1 - 1/p}\right)^{-1} \right]
\]
\[
= \left[ ?, \left(\wv_{1} \lv_{1}^{p - 1}(\wv_{1} \lv_{1}^{p} + (1 - \wv_{1})\frange^{p} )^{\frac{1}{p} - 1} \right]
\]

[worst case: pretend $\lv_{1} = \frange$ on right, leave it on left?  How loose was this?]
\[
\subseteq \left[ ?, \wv_{1}^{\frac{1}{p}} \lv_{1}^{p - 1} \frange^{1 - p} \right]
\]

This gives non-Lipschitz behavior as $\lv_{1} \to 0$, which is as expected.

TODO: FIX: minimum.

TODO: ESTIMATION THM?


\fi









\section{Data-Dependent Bounds}

\todo{Write this.}









\fi




\todo{Miscellanea}

\if 0

\section{Miscellanea}

Perverse regression example:


Take arbitrary (infinite) $\X$, $\Y = [0, 1]$.

\[
\HC_{0,1} \subseteq \X \to [0, 1]
\]

\[
\HC_{3,4} \subseteq \X to [3, 4]
\]

Loss function strictly monotonically increasing in $\abs{y - \hat{y}}$.

If $\HC_{0,1}$ is uniformly convergent, and $\HC_{3,4}$ is not, it holds that $\HC \doteq \HC_{0,1} \cup \HC_{3,4}$ is PAC-learnable (by ERM), but not uniformly convergent.

We ``cheated,'' because the codomain of $\HC$ is $[0, 1] \cup [3, 4]$, but arguably this needs to be allowed for many learning problems.

We could also define
\[
\HC' \doteq \{ \mathsmaller{\frac{1}{4}} h(x) \, | \, h \in \HC \enspace \& \ \ \ \LossFunction'(y, \hat{y}) \doteq \LossFunction(y, 4\hat{y}) \enspace,
\]
and note that $\LossFunction' \circ \HC' = \LossFunction \circ \HC$, but the codomains now align.

This is of course a ``silly'' loss function, and the asymmetry seems perverse, but we note that this asymmetric loss seems to be a requirement for tasks like \emph{weighted learning}, \emph{conditional density estimation}, and \emph{classification} given \emph{true label distributions}.



\paragraph{Polynomial versus finite sample complexity}

Exponential sample complexity in (multivariate) regression.

Suppose hypothesis class sequence $\HC$ mapping $\X \to \{0, 1\}$, such that for all $k \in \N$, $i \mapsto \VC(\HC_{i}) \in \LandauOmega(i^k)$ (i.e., the VC dimension grows superpolynomially).
Now define the \emph{regression hypothesis class}
\[
\HC_{R} \doteq \{ x \mapsto \sum_{i=0}^{\infty} 2^{-1} h_i(x) | h_i \in \HC_{i} \} \enspace,
\]
and note that $\HC_{R} \subseteq \X \to [0, 1]$.

Under any $\LossFunction$ such that $\LossFunction(y, \hat{y}) = 0$ iff $y = \hat{y}$, and $\LossFunction(a, a \pm \varepsilon)$ approaches $0$ ``sufficiently slowly''\draftnote{I need to characterize this, but any $\abs{y - \hat{y}}^{p}$ should be fine.}

$\HC_{R}$ is uniformly learnable, but with superpolynomial sample complexity.


Intuitively, each $\HC_{i}$ independently learns a single bit of the prediction.


Problem: have $0.x1\bar{0} = 0.x0\bar{1}$.
Fix: work in quaternary?  I.e., assume that in true soln, all odd bits are 0?  Or $\HC$ can enforce that?
Then firsst mistake at bit $2i$ means loss $\geq q(2^{-2i} - (2^{-2i+1} + \dots)) = \frac{1}{3 \cdot 2^{2i}}$?

If 1 to 0 mistake:
\[
\Loss(y, y_{1:2i} + \frac{1}{3 \cdot 2^{2i}}) \leq \Loss(y, \hat{y}) \leq \Loss(y, y_{1:2i})
\]
If 0 to 1 mistake:
?

In other words:
Therefore: if this regressor is UC, then so is each bit classifier (with sample complexity ?); works both ways.
But we constructed so this was not so: SC of learning bit $\ln(\frac{1}{\varepsilon^{2?}})$ is exponential?


This means
\[
\lim_{m \to \infty} SD(m) = 0
\]
but also, supposing $\VC(\HC_{i}) \geq C(4^{i})$, where %$C(4^i)$ 
$C$ is increasing, we have:

an $\varepsilon$ estimate requires a good estimate for $\HC_{i}$ where $i = \log_{4} \frac{1}{\varepsilon}$, which means
\[
m \in \LandauOmega( \frac{1}{\varepsilon} C(4^{\log_{4}(\frac{1}{\varepsilon})})) = \LandauOmega( \frac{1}{\varepsilon} C(\frac{1}{\varepsilon}) ) \enspace.
\]
Controlling the rate that $C$ increases yields arbitrary convergence rates.


This implies
\[
\epsilon \geq \frac{1}{C^{-1}(m)} ?
\]
So, take $C = \exp$, then we get an $\epsilon \geq \frac{1}{\ln(m)}$ convergence rate?


Need more assumptions on $\Loss$ though!

Need ``polynomial uniform convergence'' for PAC-learnability? It's a necessary condition? Sometimes sufficient?

Or don't assume poly SC, but instead finite?  Then poly SC is necessary for efficient PAC?

\if 0
...
Take $C$ identity. Then to re
\[
$m \in \LandauOmega( \frac{1}{\varepsilon} 4^{\log_{4}(\frac{1}{\varepsilon})}) = \LandauOmega \frac{1}{\varepsilon} 
\]


\[
SD(m)  
\approx \min(i : m \geq 4^{C(i)} )
\]
Thus need
\[
\varepsilon = 4^{-i} \approx \log_{4}(m) 
\]
\[
\log_{4}(\frac{1}{\varepsilon^2}) \in 4^(whatever)
\]
thus we can have
\[
\varepsilon = SD \in \LandauOmega(1/whatever)
\]




Need bidirectional bound? Also, loss $\leq x$ means ``not many'' mistakes in (coordinates).

Assume bits are independent in true dist?

Bound rade of this sum of losses?


SIMPLE PROOF: suppose convex loss.

Given true binary representation, $y$, e.g., $y = 0.010011011\dots$, take $y_{i}$ to be the $i$th bit of $y$ (to the right of the binary point).  Now, note that
\[
\LossFunction(y - \hat{y}) \leq \sum_{i=1}^{\infty} \LossFunction\bigl(2^{-i} (y_{i} - \hat{y}_{i})\bigr)
\]
\fi


\paragraph{Classification example?}

Take
\[
\HC \doteq \left\{ x \mapsto \begin{cases} h_{1}(x) & 1 \\ \not h_{1} \wedge h_{2} & 2 \\ \dots \bigwedge_{i=1^}{k-1} \not h_{i}(x) \wedge h_{k}(x) \\ \end{cases} \, \middle| \, \dots \right} 
\]

NOTE: ASYMM CLASSIFIER.

Can we show expo convergence?


\fi












==> paper/pacfix.tex <==



\section{COMPUTATIONAL: FIX}

\begin{lemma}[Poly-FPAC Learnability via Efficient $\varepsilon$-EMM]
\label{lemma:comp-aemm}



\end{lemma}


\cyrus{TODO: EXAMPLE: 1-FEATURE SELECTION CLASSIFIER.  OR EVEN 1D POLYNOMIAL CFIER?  CONTRAST WITH LINEAR (HYPERPLANE)?}

